Large Fluctuations in Stochastic Models of Turbulence

This dissertation discusses the intermitency phenomenon in three models of turbulence, employing analytical and numerical techniques in the analysis of stochastic processes and the probability distributions which they induce. The initial chapters present a review of the statistical theory of turbulence and of statistical theory of fields as applied to out of equilibrium physics. Two chapters of the main text investigate the RFD model and the Burgers model through the Martin-Siggia-Rose-Janssen-de Dominicis (MSRJD) functional method. An analysis of the perturbative corrections corresponding to fluctuations around the instanton in both models is undertaken. The last chapter presents a stationary one-dimensional stochastic process as a model of Lagrangian pseudo-dissipation fluctuations. It is numerically verified that this process has a lognormal probability distribution and long range power-law correlations.

==> thebib.tex <==
%%%%% ME

  @article{apolinario2019instantons,
    title={{Instantons and fluctuations in a Lagrangian model of turbulence}},
    author={Apolin{\'a}rio, G. B. and Moriconi, L. and Pereira, R. M.},
    journal={Physica A},
    volume={514},
    pages={741--757},
    year={2019},
    publisher={Elsevier}
  }

  @article{apolinario2019onset,
    title={{Onset of intermittency in stochastic Burgers hydrodynamics}},
    author={Apolin{\'a}rio, G. B. and Moriconi, L. and Pereira, R. M.},
    journal={Phys. Rev. E},
    volume={99},
    pages={033104},
    year={2019},
    publisher={APS}
  }
  
  @article{apolinario2020shotnoise,
	year = {2020},
	publisher = {{IOP} Publishing},
	volume = {2020},
	pages = {073208},
	author = {Apolin{\'{a}}rio, G. B. and Moriconi, L.},
	title = {Shot noise multifractal model for turbulent pseudo-dissipation},
	journal = {J. Stat. Mech.},
 }

  @book{schweber2012nuclear,
    title={{Nuclear forces: The making of the physicist Hans Bethe}},
    author={Schweber, S. S.},
    year={2012},
    publisher={Harvard University Press}
  }

  @article{eckert1999mathematics,
    title={{Mathematics, experiments, and theoretical physics: The early days of the Sommerfeld school}},
    author={Eckert, M.},
    journal={Physics in Perspective},
    volume={1},
    pages={238--252},
    year={1999},
    publisher={Springer}
  }

  @book{seth2010crafting,
    title={{Crafting the Quantum}},
    author={Seth, S.},
    year={2010},
    publisher={Cambridge: MIT Press}
  }

%%%%% Kolmogorov 1941

  @article{kolmogorov1941local,
    title={{The local structure of turbulence in incompressible viscous fluid for very large Reynolds numbers}},
    author={Kolmogorov, A. N.},
    journal={Cr Acad. Sci. URSS},
    volume={30},
    pages={301--305},
    year={1941}
  }

  @inproceedings{kolmogorov1941degeneration,
    title={{On degeneration (decay) of isotropic turbulence in an incompressible viscous liquid}},
    author={Kolmogorov, A. N.},
    booktitle={Dokl. Akad. Nauk SSSR},
    volume={31},
    pages={538--540},
    year={1941}
  }

  @inproceedings{kolmogorov1941dissipation,
    title={{Dissipation of energy in locally isotropic turbulence}},
    author={Kolmogorov, A. N.},
    booktitle={Akademiia Nauk SSSR Doklady},
    volume={32},
    pages={16},
    year={1941}
  }

  @article{richardson1922weather,
    title={{Weather prediction by numerical process cambridge university press}},
    author={Richardson, L. F.},
    journal={Cambridge Richardson Weather prediction by numerical process},
    volume={1922},
    year={1922}
  }

  @article{grant1962turbulence,
    title={{Turbulence spectra from a tidal channel}},
    author={Grant, H. L. and Stewart, R. W. and Moilliet, A.},
    journal={J. Fluid Mech.},
    volume={12},
    year={1962},
    publisher={Cambridge University Press}
  }
  % pages={241--268},

  @article{yeung2005,
    title={{High-Reynolds-number simulation of turbulent mixing}},
    author={Yeung, P. K. and Donzis, D. A. and Sreenivasan, K. R.},
    journal={Phys. Fluids},
    volume={17},
    pages={081703},
    year={2005},
    publisher={AIP}
  }


%%%%% Anomalous Dissipation = Zero Law

  @article{dryden1943review,
    title={{A review of the statistical theory of turbulence}},
    author={Dryden, H. L.},
    journal={Q. Appl. Math.},
    volume={1},
    pages={7--42},
    year={1943}
  }

  @article{cadot1997energy,
    title={{Energy injection in closed turbulent flows: Stirring through boundary layers versus inertial stirring}},
    author={Cadot, O. and Couder, Y. and Daerr, A. and Douady, S. and Tsinober, A.},
    journal={Phys. Rev. E},
    volume={56},
    pages={427},
    year={1997},
    publisher={APS}
  }

  @article{sreenivasan1984scaling,
    title={{On the scaling of the turbulence energy dissipation rate}},
    author={Sreenivasan, K. R.},
    journal={Phys. Fluids},
    volume={27},
    pages={1048--1051},
    year={1984},
    publisher={AIP}
  }

  @article{sreenivasan1998update,
    title={{An update on the energy dissipation rate in isotropic turbulence}},
    author={Sreenivasan, K. R.},
    journal={Phys. Fluids},
    volume={10},
    pages={528--529},
    year={1998},
    publisher={AIP}
  }

  @article{pearson2002measurements,
    title={{Measurements of the turbulent energy dissipation rate}},
    author={Pearson, B. R. and Krogstad, P.-{\AA}. and Van De Water, W.},
    journal={Phys. Fluids},
    volume={14},
    pages={1288--1290},
    year={2002},
    publisher={AIP}
  }

  @article{kaneda2003energy,
    title={{Energy dissipation rate and energy spectrum in high resolution direct numerical simulations of turbulence in a periodic box}},
    author={Kaneda, Y. and Ishihara, T. and Yokokawa, M. and Itakura, K. and Uno, A.},
    journal={Phys. Fluids},
    volume={15},
    pages={L21--L24},
    year={2003},
    publisher={AIP}
  }

  % H Nussenzveig, 2d instabilities
  @article{lacave2018asymptotic,
    title={{Asymptotic behavior of 2D incompressible ideal flow around small disks}},
    author={Lacave, C. and Lopes Filho, M. C. and Nussenzveig Lopes, H. J.},
    journal={Asymptotic Anal.},
    volume={108},
    pages={45--83},
    year={2018},
    publisher={IOS Press}
  }

  @article{nelkin1990multifractal,
    title={{Multifractal scaling of velocity derivatives in turbulence}},
    author={Nelkin, M.},
    journal={Phys. Rev. A},
    volume={42},
    pages={7226},
    year={1990},
    publisher={APS}
  }

  @phdthesis{drivas2017anomalous,
    title={{Anomalous Dissipation, Spontaneous Stochasticity \& Onsager's Conjecture}},
    author={Drivas, T. D.},
    year={2017},
    school={Johns Hopkins University}
  }

%%%%%% WEB

%https://tclf.org/sites/default/files/microsites/art-landscape/athena-tacha.html

%linux parallel, cite it

%%%%% WEB ARTICLES

  @misc{ball2014scientific,
    Author = {Ball, P.},
    Title  = "\emph{The Scientific Problem That Must Be Experienced}",
    Note   = "\url{http://nautil.us/issue/15/turbulence/the-scientific-problem-that-must-be-experienced} [Accessed: February 24th, 2020]",
    year = 2014,
  }

  @misc{ball2014feeling,
    Author = {Ball, P.},
    Title  = "\emph{ A Feeling for Flow }",
    Note   = "\url{http://philipball.blogspot.com/2014/07/a-feeling-for-flow.html}
             [Accessed: February 24th, 2020]",
    year = 2014,
  }

  @article{kemp2019leonardo,
   title={{Leonardo da Vinci’s laboratory: studies in flow}},
   volume={571},
   DOI={10.1038/d41586-019-02144-z},
   journal={Nature},
   publisher={Springer Science and Business Media LLC},
   author={Kemp, M.},
   year={2019},
   pages={322–323}
   }
   % url={http://dx.doi.org/10.1038/d41586-019-02144-z},
   % [Accessed: August 1st, 2019]

%%%%% REVIEWS

  @misc{eyink2008turbulence,
    Author = "G. L. Eyink",
    Title  = "Turbulence Theory: Course Notes",
    Note   = "\url{http://www.ams.jhu.edu/~eyink/Turbulence/notes.html}
             [Accessed: February 24th, 2020]",
    Year   = 2008,
  }

  @inbook{moriconi2008introducao,
    title={{Introdução \`{a} Teoria Estat\'{i}stica da Turbul\^{e}ncia}},
    author={L. Moriconi},
    booktitle={Turbul\^{e}ncia, volume 1 in Cole\c c\~{a}o cadernos de turbul\^{e}ncia},
    editor = {A. P. S. Freire and A. Ilha and M. J. Cola\c co},
    pages={37-97},
    publisher={ABCM, Rio de Janeiro},
    year={2008}
  }

  @book{monin2013statistical,
    title={{Statistical fluid mechanics, volume II: Mechanics of turbulence}},
    author={Monin, A. S. and Yaglom, A. M. and Lumley, J. L.},
    volume={2},
    year={2013},
    publisher={Courier Corporation}
  }
  %author={Monin, Andre{\u\i}} Sergeevich and Yaglom, Akiva M},

  @book{monin2007statistical,
    title={{Statistical Fluid Mechanics: Mechanics of Turbulence}},
    author={Monin, A. S. and Yaglom, A. M. and Lumley, J. L.},
    isbn={9780486458830},
    lccn={2006053473},
    series={Dover books on physics},
    year={2007},
    publisher={Dover Publications}
  }
  % url={https://books.google.com.br/books?id=EtTyyI4\_DvIC},

  @book{foias2001navier,
    title={{Navier-Stokes equations and turbulence}},
    author={Foias, C. and Manley, O. and Rosa, R. and Temam, R.},
    volume={83},
    year={2001},
    publisher={Cambridge University Press}
  }

  @book{kundu2008fluid,
    title={{Fluid Mechanics 4th}},
    author={Kundu, P. K. and Cohen, I. M. and Dowling, D. W.},
    year={2008},
    publisher={Elsevier}
  }

%%%%% MILLENIUM PRIZE

  @article{fefferman2006existence,
    title={{Existence and smoothness of the Navier-Stokes equation}},
    author={Fefferman, C. L.},
    journal={The Millennium Prize Problems},
    volume={57},
    pages={67},
    year={2006},
    publisher={Clay Math. Inst. Cambridge, MA}
  }

  @book{ladyzhenskaya1969mathematical,
    title={{The mathematical theory of viscous incompressible flow}},
    author={Ladyzhenskaya, O. A.},
    volume={2},
    year={1969},
    publisher={Gordon and Breach New York}
  }

%%%%% TURBULENCE AND DYNAMICAL SYSTEMS

  @article{lorenz1963,
    title={{Deterministic nonperiodic flow}},
    author={Lorenz, E. N.},
    journal={J. Atmos. Sci.},
    volume={20},
    pages={130--141},
    year={1963}
  }


  @inproceedings{landau1944problem,
    title={{On the problem of turbulence}},
    author={Landau, L. D.},
    booktitle={Dokl. Akad. Nauk USSR},
    volume={44},
    pages={311},
    year={1944}
  }

  @article{hopf1948mathematical,
    title={{A mathematical example displaying features of turbulence}},
    author={Hopf, E.},
    journal={Commun. Pur. Appl. Math.},
    volume={1},
    pages={303--322},
    year={1948},
    publisher={Wiley Online Library}
  }

%%%%% FUNCTIONAL

  @article{hopf1952statistical,
    title={{Statistical hydromechanics and functional calculus}},
    author={Hopf, E.},
    journal={J. Ration. Mech. Anal.},
    volume={1},
    pages={87--123},
    year={1952},
    publisher={JSTOR}
  }

  @article{kraichnan1958higher,
    title={{Higher order interactions in homogeneous turbulence theory}},
    author={Kraichnan, R. H.},
    journal={Phys. Fluids},
    volume={1},
    pages={358--359},
    year={1958},
    publisher={AIP}
  }

  @article{lewis1962space,
    title={{A space-time functional formalism for turbulence}},
    author={Lewis, R. M. and Kraichnan, R. H.},
    journal={Commun. Pur. Appl. Math.},
    volume={15},
    pages={397--411},
    year={1962},
    publisher={Wiley Online Library}
  }

  @article{tatarskii1962application,
    title={{Application of quantum field theory methods to the problem of degeneration of homogeneous turbulence}},
    author={Tatarskii, V. I.},
    journal={Sov. Phys. JETP},
    volume={15},
    year={1962}
  }

  @article{wyld1961formulation,
    title={{Formulation of the theory of turbulence in an incompressible fluid}},
    author={Wyld Jr, H. W.},
    journal={Ann. Phys.},
    volume={14},
    pages={143--165},
    year={1961},
    publisher={Elsevier}
  }

  @article{kraichnan1961dynamics,
    title={{Dynamics of nonlinear stochastic systems}},
    author={Kraichnan, R. H.},
    journal={J. Math. Phys.},
    volume={2},
    pages={124--148},
    year={1961},
    publisher={AIP}
  }

  @article{falkovich19932d,
  title={{Is 2D turbulence a conformal turbulence?}},
  author={Falkovich, G. and Hanany, A.},
  journal={Phys. Rev. Lett.},
  volume={71},
  pages={3454},
  year={1993},
  publisher={APS}
  }

  @article{falkovich1994universal,
  title={{Universal direct cascade in two-dimensional turbulence}},
  author={Falkovich, G. and Lebedev, V.},
  journal={Phys. Rev. E},
  volume={50},
  pages={3883},
  year={1994},
  publisher={APS}
  }

  @article{benzi1995conformal,
  title={{Conformal field theory and direct numerical simulation of two-dimensional turbulence}},
  author={Benzi, R. and Legras, B. and Parisi, G. and Scardovelli, R.},
  journal={Europhys. Lett.)},
  volume={29},
  pages={203},
  year={1995},
  publisher={IOP Publishing}
  }

  @article{polyakov1993theory,
  title={{The theory of turbulence in two dimensions}},
  author={Polyakov, A. M.},
  journal={Nucl. Phys. B},
  volume={396},
  pages={367--385},
  year={1993},
  publisher={Elsevier}
  }

  @article{onsager1953fluctuations,
  title={{Fluctuations and irreversible processes}},
  author={Onsager, L. and Machlup, S.},
  journal={Phys. Rev.},
  volume={91},
  pages={1505},
  year={1953},
  publisher={APS}
  }

  @article{phythian1977functional,
  title={{The functional formalism of classical statistical dynamics}},
  author={Phythian, R.},
  journal={J. Phys. A},
  volume={10},
  pages={777},
  year={1977},
  publisher={IOP Publishing}
  }

  @article{fournier1978infinite,
  title={{Infinite-dimensional turbulence}},
  author={Fournier, J. D. and Frisch, U. and Rose, H. A.},
  journal={J. Phys. A},
  volume={11},
  pages={187},
  year={1978},
  publisher={IOP Publishing}
  }

  @article{fournier1983remarks,
  title={{Remarks on the renormalization group in statistical fluid dynamics}},
  author={Fournier, J.-D. and Frisch, U.},
  journal={Phys. Rev. A},
  volume={28},
  pages={1000},
  year={1983},
  publisher={APS}
  }

  @article{canet2016fully,
    title={{Fully developed isotropic turbulence: Nonperturbative renormalization group formalism and fixed-point solution}},
    author={Canet, L. and Delamotte, B. and Wschebor, N.},
    journal={Phys. Rev. E},
    volume={93},
    pages={063101},
    year={2016},
    publisher={APS}
  }

  @article{tarpin2018stationary,
    title={{Stationary, isotropic and homogeneous two-dimensional turbulence: a first non-perturbative renormalisation group approach}},
    author={Tarpin, M. and Canet, L. and Pagani, C. and Wschebor, N.},
    journal={J. Phys. A},
    year={2018},
    publisher={IOP Publishing}
  }

  @article{canet2017spatiotemporal,
    title={{Spatiotemporal velocity-velocity correlation function in fully developed turbulence}},
    author={Canet, L. and Rossetto, V. and Wschebor, N. and Balarac, G.},
    journal={Phys. Rev. E},
    volume={95},
    pages={023107},
    year={2017},
    publisher={APS}
  }

  @article{langouche1979,
    title={{Functional integral methods for stochastic fields}},
    author={Langouche, F. and Roekaerts, D. and Tirapegui, E.},
    journal={Physica A},
    volume={95},
    pages={252--274},
    year={1979},
    publisher={Elsevier}
  }

  @article{jensen1981functional,
    title={{Functional integral approach to classical statistical dynamics}},
    author={Jensen, R. V.},
    journal={J. Stat. Phys.},
    volume={25},
    pages={183--210},
    year={1981},
    publisher={Springer}
  }

  @article{martin1973,
    title = {{Statistical Dynamics of Classical Systems}},
    author = {P. C. Martin and E. D. Siggia and H. A. Rose},
    journal = {Phys. Rev. A},
    volume = {\textbf{8}},
    issue = {1},
    pages = {423},
    year = 1973,
  }

  @article{dominicis1976,
    author = {C. de Dominicis},
    title = {{Techniques de Renormalization de la Theorie des Champs et Dynamique des Phenomenes Critques}},
    journal = {J. Phys. Colloques},
    year = 1976,
    volume = "\textbf{37}",
    pages = "247",
  }

  @article{janssen1976,
  title={{On a Lagrangean for classical field dynamics and renormalization group calculations of dynamical critical properties}},
  author={Janssen, H.-K.},
  journal={Z. Phys. B Con. Mat.},
  volume={23},
  pages={377--380},
  year={1976},
  publisher={Springer}
  }

%%%%% VIDEOS

  @misc{schaal2015kelvin,
    Author = "K. Schaal",
    Title  = "Kelvin-Helmholtz instability - Discontinuous Galerkin hydrodynamics",
    Note   = "\url{https://www.youtube.com/watch?v=cTRQP6DSaqA}
             [Accessed: February 24th, 2020]",
    Year   = 2015,
  }

  @misc{swiss2009technorama,
    Author = {T. R. Eisenberg},
    Title  = "Technorama Facade by Ned Khan",
    Note   = "\url{https://www.swiss-miss.com/2009/05/technorama-facade-by-ned-khan.html}
             [Accessed: February 24th, 2020]",
    Year   = 2009,
  }

%%%%% OTHERS

  @article{zeff2003,
   author={Zeff, B. W. and Lan\-ter\-man, D. D., and Mc\-A\-llis\-ter, R. and Roy, R. and Kos\-te\-lich, E. J. and La\-throp, D. P.},
   title={{Measuring intense rotation and dissipation in turbulent flows}},
   journal={Nature},
   pages=146,
   year=2003
  }

  @article{WallaceEF,
   author="V. Vukoslavcevic and N. Beratlis and E. Balaras and J. M. Wallace and O. Sun",
   title={{On the spatial resolution of velocity and velocity gradient-based turbulence statistics measured with multi-sensor hot-wire probes}},
   journal="Exp. Fluids",
   pages=109,
   year=2009
  }

  @article{wallace2009,
    author={J. Wallace},
    title={{Twenty years of experimental and direct numerical simulation access to the velocity gradient tensor: What have we learned about turbulence?}},
    journal={Phys. Fluids},
    pages={021301},
    year={2009}
  }

  @article{Martin98,
  author="J. Martin and C. Dopazo and L. Valino",
  title={{ Dynamics of velocity gradient invariants in turbulence: restricted Euler and linear diffusion models}},
  journal="Phys. Fluids",
  pages=2012,
  year=1998
  }

  @article{girimaji90diffusion,
  author={Girimaji, S. S. and Pope, S. B.},
  title={{A diffusion model for velocity gradients in turbulence}},
  journal="Phys. Fluids A",
  pages=242,
  year=1990
  }

  @article{Chertkov99,
  author="M. Chertkov and A. Pumir and B. I. Shraiman",
  title={{Lagrangian tetrad dynamics and the phenomenology of turbulence}},
  journal="Phys. Fluids",
  pages=2394,
  year=1999
  }

  @article{Jeong2003,
  author="E. Jeong and S. S. Girimaji",
  title={{Velocity-gradient dynamics in turbulence: effect of viscosity and forcing}},
  journal="Comput. Fluid Dyn.",
  pages=421,
  year=2003
  }

  @article{vukoslav91,
    title={{The velocity and vorticity vector fields of a turbulent boundary layer}},
    author={P. Vukoslavcevic and J. Wallace and J. L. Balint},
    journal={J. Fluid Mech.},
    volume={\textbf{228}},
    pages={25},
    year={1991},
  }

  @misc{LeoBouchet,
   author    = {Grigorio, L. S. and Bouchet, F. and Pereira, R. M. and Chevillard, L.},
   title     = {Instantons in a Lagrangian model of turbulence},
   archivePrefix = {arXiv},
   eprint        = {1608.07332},
   primaryClass  = {flu-dyn}
  }

  @book{TsinoberInformal,
    title={{An Informal Conceptual Introduction to Turbulence: Second Edition of An Informal Introduction to Turbulence}},
    author={A. Tsinober},
    year={2009},
    publisher={Springer Netherlands}
  }

  @article{MoriconiPereiraPRE,
    title = {Vorticity statistics and the time scales of turbulent strain},
    author = {L. Moriconi  and R. M. Pereira},
    journal = {Phys. Rev. E},
    volume = {\textbf{88}},
    issue = {1},
    pages = {013005},
    year = {2013}
    }

  @article{sreenivasan1997phenomenology,
    title={{The phenomenology of small-scale turbulence}},
    author={Sreenivasan, K. R. and Antonia, R. A.},
    journal={Annu. Rev. Fluid Mech.},
    volume={29},
    pages={435--472},
    year={1997},
    publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
  }

  @article{dubrulle2019beyond,
    title={{Beyond Kolmogorov cascades}},
    author={Dubrulle, B.},
    journal={J. Fluid Mech.},
    volume={867},
    year={2019},
    publisher={Cambridge University Press}
  }

  @article{WallaceVukoslav2010,
    author="J. M. Wallace and P. V. Vukoslavcevic",
    title={{Experimental Measurement of the Velocity Gradient Tensor}},
    journal={Annu. Rev. of Fluid Mech.},
    pages={157},
    year={2010}
  }

  @article{KatzSheng2010,
    author={Katz, J. and Sheng, J.},
    title={{Applications of Holography in Fluid Mechanics and Particle Dynamics}},
    journal={Annu. Rev. Fluid Mech.},
    pages={531},
    year={2010}
  }

  @book{HolmesLumley,
    title={{Turbulence, Coherent Structures, Dynamical Systems and Symmetry}},
    author={P. Holmes and J. L. and Lumley and G. Berkooz},
    series={Cambridge Monographs on Mechanics},
    year={1998},
    publisher={Cambridge University Press}
  }

  @article{cardesa2017turbulent,
    title={{The turbulent cascade in five dimensions}},
    author={Cardesa, J. I. and Vela-Martin, A. and Jim{\'e}nez, J.},
    journal={Science},
    pages={eaan7933},
    year={2017},
    publisher={American Association for the Advancement of Science}
  }
  %author={Cardesa, J. I. and Vela-Mart{\'\i}n, A. and Jim{\'e}nez, J.},

  @article{bernard1998scaling,
    title={{Scaling and exotic regimes in decaying Burgers turbulence}},
    author={Bernard, D. and Gawedzki, K.},
    journal={J. Phys. A},
    volume={31},
    pages={8735},
    year={1998},
    publisher={IOP Publishing}
  }

  @article{falkovich2001particles,
    title={{Particles and fields in fluid turbulence}},
    author={Falkovich, G. and Gawedzki, K. and Vergassola, M.},
    journal={Rev. Mod. Phys.},
    volume={73},
    pages={913},
    year={2001},
    publisher={APS}
  }

  @article{gioia2010spectral,
    title={{Spectral theory of the turbulent mean-velocity profile}},
    author={Gioia, G. and Guttenberg, N. and Goldenfeld, N. and Chakraborty, P.},
    journal={Phys. Rev. Lett.},
    volume={105},
    pages={184501},
    year={2010},
    publisher={APS}
  }

  @article{yakhot2017emergence,
    title={{Emergence of multiscaling in a random-force stirred fluid}},
    author={Yakhot, V. and Donzis, D.},
    journal={Phys. Rev. Lett.},
    volume={119},
    pages={044501},
    year={2017},
    publisher={APS}
  }

  @article{yakhot1992renormalization,
    title={{The renormalization group, the $\varepsilon$-expansion and derivation of turbulence models}},
    author={Yakhot, V. and Smith, L. M.},
    journal={J. Sci. Comput.},
    volume={7},
    pages={35--61},
    year={1992},
    publisher={Springer}
  }

  @article{schumacher2007asymptotic,
    title={{Asymptotic exponents from low-Reynolds-number flows}},
    author={Schumacher, J. and Sreenivasan, K. R. and Yakhot, V.},
    journal={New J. Phys.},
    volume={9},
    pages={89},
    year={2007},
    publisher={IOP Publishing}
  }

  @article{yakhot2003pressure,
    title={{Pressure--velocity correlations and scaling exponents in turbulence}},
    author={Yakhot, V.},
    journal={J. Fluid Mech.},
    volume={495},
    pages={135--143},
    year={2003},
    publisher={Cambridge University Press}
  }

  @article{yakhot2014reynolds,
    title={{Reynolds number of transition and self-organized criticality of strong turbulence}},
    author={Yakhot, V.},
    journal={Phys. Rev. E},
    volume={90},
    pages={043019},
    year={2014},
    publisher={APS}
  }

  @article{friedrich2018,
    title={{Multiscale velocity correlations in turbulence and Burgers turbulence: Fusion rules, Markov processes in scale, and multifractal predictions}},
    author={Friedrich, J. and Margazoglou, G. and Biferale, L. and Grauer, R.},
    journal={Phys. Rev. E},
    volume={98},
    pages={023104},
    year={2018},
    publisher={APS}
  }

  @article{ishihara2009,
    title={{Study of high--Reynolds number isotropic turbulence by direct numerical simulation}},
    author={Ishihara, T. and Gotoh, T. and Kaneda, Y.},
    journal={Annu. Rev. Fluid Mech.},
    volume={41},
    year={2009},
    publisher={Annual Reviews}
  }

  @article{benzi2010inertial,
    title={{Inertial range Eulerian and Lagrangian statistics from numerical simulations of isotropic turbulence}},
    author={Benzi, R. and Biferale, L. and Fisher, R. and Lamb, D. Q. and Toschi, F.},
    journal={J. Fluid Mech.},
    volume={653},
    year={2010},
    publisher={Cambridge University Press}
  }


  @article{sinhuber2017dissipative,
    title={{Dissipative effects on inertial-range statistics at high Reynolds numbers}},
    author={Sinhuber, M. and Bewley, G. P. and Bodenschatz, E.},
    journal={Phys. Rev. Lett.},
    volume={119},
    year={2017},
    publisher={APS}
  }

  @article{iyer2017reynolds,
    title={{Reynolds number scaling of velocity increments in isotropic turbulence}},
    author={Iyer, K. P. and Sreenivasan, K. R. and Yeung, P. K.},
    journal={Phys. Rev. E},
    volume={95},
    year={2017},
    publisher={APS}
  }


  @article{reinke2018universal,
    title={{On universal features of the turbulent cascade in terms of non-equilibrium thermodynamics}},
    author={Reinke, N. and Fuchs, A. and Nickelsen, D. and Peinke, J.},
    journal={J. Fluid Mech.},
    volume={848},
    pages={117--153},
    year={2018},
    publisher={Cambridge University Press}
  }

  @article{mandelbrot1974intermittent,
    title={{Intermittent turbulence in self-similar cascades: divergence of high moments and dimension of the carrier}},
    author={Mandelbrot, B. B.},
    journal={J. Fluid Mech.},
    volume={62},
    pages={331--358},
    year={1974},
    publisher={Cambridge University Press}
  }

  @article{debue2018experimental,
    title={{Experimental test of the crossover between the inertial and the dissipative range in a turbulent swirling flow}},
    author={Debue, P. and Kuzzay, D. and Saw, E.-W. and Daviaud, F. and Dubrulle, B. and Canet, L. and Rossetto, V. and Wschebor, N.},
    journal={Phys. Rev. Fluids},
    volume={3},
    pages={024602},
    year={2018},
    publisher={APS}
  }

  %%%%% Large Deviation Theory

  @article{freidlin2004random,
    title={{Random perturbations of dynamical systems and diffusion processes with conservation laws}},
    author={Freidlin, M. and Weber, M.},
    journal={Probab. Theory Rel.},
    volume={128},
    pages={441--466},
    year={2004},
    publisher={Springer}
  }

  %%%%%

  @article{chevillard2007intermittency,
    title={{Intermittency and universality in a Lagrangian model of velocity gradients in three-dimensional turbulence}},
    author={Chevillard, L. and Meneveau, C.},
    journal={C. R. M{\'e}canique},
    volume={335},
    pages={187--193},
    year={2007},
    publisher={Elsevier}
  }

  % short journal names, refs stopped here

  @article{onsager1949statistical,
    title={{Statistical hydrodynamics}},
    author={Onsager, L.},
    journal={Nuovo Cimento},
    volume={6},
    pages={279--287},
    year={1949},
    publisher={Springer}
  }

  @article{taylor1938spectrum,
    title={{The spectrum of turbulence}},
    author={Taylor, G. I.},
    journal={Proc. R. Soc. Lon. Ser.-A},
    volume={164},
    pages={476--490},
    year={1938},
    publisher={The Royal Society}
  }

  @book{kahane1993some,
    title={{Some random series of functions}},
    author={Kahane, J.-P.},
    volume={5},
    year={1993},
    publisher={Cambridge University Press}
  }

  @article{ruelle1982large,
    title={{Large volume limit of the distribution of characteristic exponents in turbulence}},
    author={Ruelle, D.},
    journal={Commun. Math. Phys.},
    volume={87},
    pages={287--302},
    year={1982},
    publisher={Springer}
  }

  @article{vassilicos2015dissipation,
    title={{Dissipation in turbulent flows}},
    author={Vassilicos, J. C.},
    journal={Annu. Rev. Fluid Mech.},
    volume={47},
    pages={95--114},
    year={2015},
    publisher={Annual Reviews}
  }

  @article{bitane2013geometry,
    title={{Geometry and violent events in turbulent pair dispersion}},
    author={Bitane, R. and Homann, H. and Bec, J.},
    journal={J. Turbul.},
    volume={14},
    pages={23--45},
    year={2013},
    publisher={Taylor \& Francis}
  }

  @article{morozov1984langevin,
    title={{On the Langevin formalism for nonlinear and nonequilibrium hydrodynamic fluctuations}},
    author={Morozov, V. G.},
    journal={Physica A},
    volume={126},
    pages={443--460},
    year={1984},
    publisher={Elsevier}
  }

  @article{anselmet1984high,
    title={{High-order velocity structure functions in turbulent shear flows}},
    author={Anselmet, F. and Gagne, Y. and Hopfinger, E. J. and Antonia, R. A.},
    journal={J. Fluid Mech.},
    volume={140},
    pages={63--89},
    year={1984},
    publisher={Cambridge University Press}
  }

  @article{bernard1998slow,
    title={{Slow modes in passive advection}},
    author={Bernard, D. and Gawedzki, K. and Kupiainen, A.},
    journal={J. Stat. Phys.},
    volume={90},
    pages={519--569},
    year={1998},
    publisher={Springer}
  }

  @article{aurell1992multifractal,
    title={{On the multifractal properties of the energy dissipation derived from turbulence data}},
    author={Aurell, E. and Frisch, U. and Lutsko, J. and Vergassola, M.},
    journal={J. Fluid Mech.},
    volume={238},
    pages={467--486},
    year={1992},
    publisher={Cambridge University Press}
  }

  @article{dryden1941isotropic,
  title={{Isotropic turbulence in theory and experiment}},
  author={Dryden, H. L.},
  journal={T. von Karman Anniv},
  volume={85},
  year={1941}
  }

  @article{meneveau1987multifractal,
    title={{The multifractal spectrum of the dissipation field in turbulent flows}},
    author={Meneveau, C. and Sreenivasan, K. R.},
    journal={Nucl. Phys. B},
    volume={2},
    pages={49--76},
    year={1987},
    publisher={Elsevier}
  }

  @article{meneveau1991multifractal,
    title={{The multifractal nature of turbulent energy dissipation}},
    author={Meneveau, C. and Sreenivasan, K. R.},
    journal={J. Fluid Mech.},
    volume={224},
    pages={429--484},
    year={1991},
    publisher={Cambridge University Press}
  }

  @book{einstein1956investigations,
    title={{Investigations on the Theory of the Brownian Movement}},
    author={Einstein, A.},
    year={1956},
    publisher={Courier Corporation}
  }

  @article{langevin1908theorie,
    title={{Sur la th{\'e}orie du mouvement brownien}},
    author={Langevin, P.},
    journal={C. R. Acad. Sci. Paris.},
    volume={146},
    pages={530--533},
    year={1908}
  }

  @misc{cugliandolo2018building,
    title={Building a path-integral calculus},
    author={Cugliandolo, L. F. and Lecomte, V. and Van Wijland, F.},
    archivePrefix = {arXiv},
    eprint        = {1806.09486},
    primaryClass  = {cond-mat.stat-mech},
    year = {2018}
  }

  @article{nakazato1990symmetries,
    title={{Symmetries in stochastic quantization and Ito-Stratonovich related interpretation}},
    author={Nakazato, H. and Okano, K. and Schulke, L. and Yamanaka, Y.},
    journal={Nucl. Phys. B},
    volume={346},
    pages={611--631},
    year={1990},
    publisher={Elsevier}
  }
  % in fact, Sch{\"u}lke

  @article{galanti2004turbulence,
    title={{Is turbulence ergodic?}},
    author={Galanti, B. and Tsinober, A.},
    journal={Phys. Lett. A},
    volume={330},
    pages={173--180},
    year={2004},
    publisher={Elsevier}
  }

  @book{feynman2011feynmanvol2,
    title={{The Feynman Lectures on Physics}},
    author={Feynman, R. P. and Leighton, R. B. and Sands, M.},
    volume={II},
    year={2011},
    publisher={Basic books}
  }

  @article{taylor1938production,
    title={{Production and dissipation of vorticity in a turbulent fluid}},
    author={Taylor, G. I.},
    journal={Proc. R. Soc. Lon. Ser.-A},
    volume={164},
    pages={15--23},
    year={1938},
    publisher={The Royal Society London}
  }

  @article{ruelle1981differentiable,
    title={{Differentiable dynamical systems and the problem of turbulence}},
    author={Ruelle, D.},
    journal={B. Am. Math. Soc.},
    volume={5},
    pages={29--42},
    year={1981}
  }

  % Ergodic theory and birkhoff's theorem

  @book{cornfeld2012ergodic,
    title={{Ergodic theory}},
    author={Cornfeld, I. P. and Fomin, S. V. and Sinai, Y. G.},
    volume={245},
    year={2012},
    publisher={Springer Science \& Business Media}
  }

  @inproceedings{sinai1963,
    title={{On the foundations of the ergodic hypothesis for a dynamical system of statistical mechanics}},
    author={Sinai, Y. G.},
    booktitle={Doklady Akademii Nauk},
    volume={153},
    pages={1261--1264},
    year={1963},
    organization={Russian Academy of Sciences}
  }

  @book{dubois1999,
    title={{Dynamic multilevel methods and the numerical simulation of turbulence}},
    author={Dubois, T. and Jauberteau, F. and Temam, R.},
    year={1999},
    publisher={Cambridge University Press}
  }

  @book{fursikov1988,
    title={{Mathematical problems of statistical hydrodynamics}},
    author={Fursikov, A. W. and Vishik, M. I.},
    year={1988},
    publisher={Kluwer Academic Publisher, Dordrecht}
  }

  @article{ruelle1971,
    title={{On the nature of turbulence}},
    author={Ruelle, D. and Takens, F.},
    journal={Les rencontres physiciens-math{\'e}maticiens de Strasbourg-RCP25},
    volume={12},
    pages={1--44},
    year={1971}
  }



%%%%% LAGRANGIAN CHAPTER

  @article{borgas1993multifractal,
    title={{The multifractal Lagrangian nature of turbulence}},
    author={Borgas, M. S.},
    journal={Philos. T. R. Soc. Lond.},
    volume={342},
    pages={379--411},
    year={1993},
    publisher={The Royal Society London}
  }

  @article{ott2000experimental,
    title={{An experimental investigation of the relative diffusion of particle pairs in three-dimensional turbulent flow}},
    author={Ott, S. and Mann, J.},
    journal={J. Fluid Mech.},
    volume={422},
    pages={207--223},
    year={2000},
    publisher={Cambridge University Press}
  }

  @article{biferale2004multifractal,
    title={{Multifractal statistics of Lagrangian velocity and acceleration in turbulence}},
    author={Biferale, L. and Boffetta, G. and Celani, A. and Devenish, B. J. and Lanotte, A. and Toschi, F.},
    journal={Phys. Rev. Lett.},
    volume={93},
    pages={064502},
    year={2004},
    publisher={APS}
  }

  @article{hartman2002ordinary,
    title={{Ordinary Differential Equations, Classics in Applied Mathematics}},
    author={Hartman, P.},
    journal={Society for Industrial and Applied Mathematics (SIAM), Philadelphia, PA},
    volume={38},
    year={2002}
  }

  @article{richardson1926atmospheric,
    title={{Atmospheric diffusion shown on a distance-neighbour graph}},
    author={Richardson, L. F.},
    journal={Proc. R. Soc. Lon. Ser.-A},
    volume={110},
    pages={709--737},
    year={1926},
    publisher={The Royal Society London}
  }

  @article{das2019reynolds,
    title={{On the Reynolds number dependence of velocity-gradient structure and dynamics}},
    author={Das, R. and Girimaji, S. S.},
    journal={J. Fluid Mech.},
    volume={861},
    pages={163--179},
    year={2019},
    publisher={Cambridge University Press}
  }

  @article{watteaux2019time,
    title={{On the time scales and structure of Lagrangian intermittency in homogeneous isotropic turbulence}},
    author={Watteaux, R. and Sardina, G. and Brandt, L. and Iudicone, D.},
    journal={J. Fluid Mech.},
    volume={867},
    pages={438--481},
    year={2019},
    publisher={Cambridge University Press}
  }

  @article{meneveau2011lagrangian,
    title={{Lagrangian dynamics and models of the velocity gradient tensor in turbulent flows}},
    author={Meneveau, C.},
    journal={Annu. Rev. Fluid Mech.},
    volume={43},
    pages={219--245},
    year={2011},
    publisher={Annual Reviews}
  }

  @article{cantwell1992exact,
    title={{Exact solution of a restricted Euler equation for the velocity gradient tensor}},
    author={Cantwell, B. J.},
    journal={Phys. Fluids A},
    volume={4},
    pages={782--793},
    year={1992},
    publisher={AIP}
  }

  @article{ashurst1987alignment,
    title={{Alignment of vorticity and scalar gradient with strain rate in simulated Navier--Stokes turbulence}},
    author={Ashurst, W. T. and Kerstein, A. R. and Kerr, R. M. and Gibson, C. H.},
    journal={Phys. Fluids},
    volume={30},
    pages={2343--2353},
    year={1987},
    publisher={AIP}
  }

  @article{constantin2008stochastic,
    title={{A stochastic Lagrangian representation of the three-dimensional incompressible Navier-Stokes equations}},
    author={Constantin, P. and Iyer, G.},
    journal={Commun. Pur. Appl. Math.},
    volume={61},
    pages={330--345},
    year={2008},
    publisher={Wiley Online Library}
  }

  @book{arnold1992ordinary,
    title={{Ordinary Differential Equations}},
    author={Arnold, V. I.},
    isbn={9783540548133},
    lccn={91044188},
    series={Springer Textbook},
    year={1992},
    publisher={Springer Berlin Heidelberg}
  }

  @article{sawford2001turbulent,
    title={{Turbulent relative dispersion}},
    author={Sawford, B.},
    journal={Annu. Rev. Fluid Mech.},
    volume={33},
    pages={289--317},
    year={2001},
    publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
  }

  @book{kunita1997stochastic,
    title={{Stochastic flows and stochastic differential equations}},
    author={Kunita, H.},
    volume={24},
    year={1997},
    publisher={Cambridge university press}
  }

  @article{taylor1922diffusion,
    title={{Diffusion by continuous movements}},
    author={Taylor, G. I.},
    journal={P. Lond. Math. Soc.},
    volume={2},
    pages={196--212},
    year={1922},
    publisher={Wiley Online Library}
  }

  @article{biferale2006lagrangian,
    title={{Lagrangian statistics in fully developed turbulence}},
    author={Biferale, L. and Boffetta, G. and Celani, A. and Lanotte, A. and Toschi, F.},
    journal={J. Turbul.},
    pages={N6},
    year={2006},
    publisher={Taylor \& Francis}
  }

  @article{mordant2001measurement,
    title={{Measurement of Lagrangian velocity in fully developed turbulence}},
    author={Mordant, N. and Metz, P. and Michel, O. and Pinton, J.-F.},
    journal={Phys. Rev. Lett.},
    volume={87},
    pages={214501},
    year={2001},
    publisher={APS}
  }

  @article{boffetta1999relative,
    title={{Relative dispersion in fully developed turbulence: Lagrangian statistics in synthetic flows}},
    author={Boffetta, G. and Celani, A. and Crisanti, A. and Vulpiani, A.},
    journal={Europhys. Lett.},
    volume={46},
    pages={177},
    year={1999},
    publisher={IOP Publishing}
  }

  @article{thomson2005particle,
    title={{Particle pair separation in kinematic simulations}},
    author={Thomson, D. J. and Devenish, B. J.},
    journal={J. Fluid Mech.},
    volume={526},
    pages={277--302},
    year={2005},
    publisher={Cambridge University Press}
  }

  @article{elliott1996pair,
    title={{Pair dispersion over an inertial range spanning many decades}},
    author={Elliott Jr., F. W. and Majda, A. J.},
    journal={Phys. Fluids},
    volume={8},
    pages={1052--1060},
    year={1996},
    publisher={AIP}
  }

%%%%% MULTIFRACTAL MODEL

  @inproceedings{frisch1985singularity,
    title={{On the singularity structure of fully developed turbulence}},
    author={Frisch, U. and Parisi, G.},
    booktitle={Turbulence and predictability in geophysical fluid dynamics and climate dynamics},
    editor={Ghil, M. and Benzi, R. and Parisi, G.},
    date={1985},
    booktitleaddon = {Proceedings of the International School of Physics E. Fermi},
    eventdate = {1983},
    venue = {Varenna, Italy},

  }

  @article{kestener2004generalizing,
    title={{Generalizing the wavelet-based multifractal formalism to random vector fields: application to three-dimensional turbulence velocity and vorticity data}},
    author={Kestener, P. and Arneodo, A.},
    journal={Phys. Rev. Lett.},
    volume={93},
    pages={044501},
    year={2004},
    publisher={APS}
  }

  @article{arneodo2008wavelet,
    title={{Wavelet-based multifractal analysis}},
    author={Arneodo, A. and Audit, B. and Kestener, P. and Roux, S.},
    journal={Scholarpedia},
    volume={3},
    pages={4103},
    year={2008}
  }

  @article{muzy1991wavelets,
    title={{Wavelets and multifractal formalism for singular signals: Application to turbulence data}},
    author={Muzy, J.-F. and Bacry, E. and Arneodo, A.},
    journal={Phys. Rev. Lett.},
    volume={67},
    pages={3515},
    year={1991},
    publisher={APS}
  }

  @article{parisi1985turbulence,
    title={{Turbulence and predictability in geophysical fluid dynamics}},
    author={Parisi, G.},
    journal={Proc. Intern. School of Physics' Enrico Fermi', 1983, Varenna, Italy},
    year={1985},
    publisher={North-Holland}
  }

%%%%% GALLERY

  @book{leal2003gallery,
    title={{A Gallery of Fluid Motion}},
    author={Leal, L. G. and Steen, P. H. and Samimy, M. and Breuer, K. S.},
    year={2003},
    publisher={Cambridge University Press}
  }

  @book{van1982album,
    title={{An album of fluid motion}},
    author={Van Dyke, M.},
    year={1982},
    publisher={Parabolic Press Stanford}
  }

  @misc{gfm,
      Author={{AMERICAN PHYSICAL SOCIETY}},
      Title  = "\emph{Gallery of Fluid Motion}",
      Note   = "\url{https://gfm.aps.org/} [Accessed: February 24th, 2020]",
      year = {2019},
  }

  @book{clarke2012water,
    title={{Water and art}},
    author={Clarke, D.},
    year={2012},
    publisher={Reaktion Books}
  }

  @book{leonardocodex,
    title={{Leonardo da Vinci's Codex Leicester: A New Edition (Volume 1)}},
    author={Laurenza, D. and Kemp, M.},
    year=2019,
    publisher={Oxford University Press}
  }

%%%%% NUMERICAL VALUES

  @misc{visc-water,
        Author = {{EN\-GI\-NEER\-ING TOOL\-BOX}},
        Title  = "\emph{Water - Dynamic and Kinematic Viscosity}",
        Note   = "\url{https://www.engineeringtoolbox.com/water-dynamic-kinematic-viscosity-d_596.html} [Accessed: February 24th, 2020]",
        year = {2004},
    }

  @misc{visc-air,
        Author = {{ENGINEERING TOOLBOX}},
        Title  = "\emph{Air - Dynamic and Kinematic Viscosity }",
        Note   = "\url{https://www.engineeringtoolbox.com/air-absolute-kinematic-viscosity-d_601.html}   [Accessed: February 24th, 2020]",
        year = {2003},
    }

%%%%% HISTORY

  @article{rott1990note,
    title={{Note on the history of the Reynolds number}},
    author={Rott, N.},
    journal={Annu. Rev. Fluid Mech.},
    volume={22},
    pages={1--12},
    year={1990},
    publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
  }

%%%%% WAVELETS

  @article{farge1992wavelet,
    title={{Wavelet transforms and their applications to turbulence}},
    author={Farge, M.},
    journal={Annu. Rev. Fluid Mech.},
    volume={24},
    pages={395--458},
    year={1992},
    publisher={Annual reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
  }

%%%%% SIMULATIONS

  @book{gottlieb1977numerical,
    title={{Numerical analysis of spectral methods: theory and applications}},
    author={Gottlieb, D. and Orszag, S. A.},
    volume={26},
    year={1977},
    publisher={Siam}
  }

%%%% SINGULARITIES

  @incollection{scheffer1976turbulence,
    title={{Turbulence and Hausdorff dimension}},
    author={Scheffer, V.},
    booktitle={Turbulence and Navier Stokes Equations},
    pages={174--183},
    year={1976},
    publisher={Springer}
  }

  @article{scheffer1980navier,
    title={{The Navier-Stokes equations on a bounded domain}},
    author={Scheffer, V.},
    journal={Commun. Math. Phys.},
    volume={73},
    pages={1--42},
    year={1980},
    publisher={Springer}
  }

%%%%% EXPERIMENTAL DATA

  @article{sreenivasan1995universality,
    title={{On the universality of the Kolmogorov constant}},
    author={Sreenivasan, K. R.},
    journal={Phys. Fluids},
    volume={7},
    year={1995},
    publisher={AIP}
  }

%%%%% BROWNIAN MOTION
% all of these should be reviewed for correctness, accents,

@book{thiele1880,
  title={{Sur la compensation de quelques erreurs quasi-syst{\'e}matiques par la m{\'e}thode des moindres carr{\'e}s}},
  author={Thiele, T. N.},
  year={1880},
  publisher={CA Reitzel, Copenhagen}
}

@incollection{jarrow2004,
  title={{A short history of stochastic integration and mathematical finance: the early years, 1880--1970}},
  author={Jarrow, R. and Protter, P.},
  booktitle={A festschrift for Herman Rubin},
  pages={75--91},
  year={2004},
  publisher={Institute of Mathematical Statistics}
}

@article{brown1828,
  title={{Mikroskopische Beobachtungen {\"u}ber die im Pollen der Pflanzen enthaltenen Partikeln, und {\"u}ber das allgemeine Vorkommen activer Molec{\"u}le in organischen und unorganischen K{\"o}rpern}},
  author={Brown, R.},
  journal={Ann. Phys.},
  volume={90},
  pages={294--313},
  year={1828},
  publisher={Wiley Online Library}
}

@article{einstein1905,
  title={{On the movement of small particles suspended in station-
ary liquid demanded by the molecular-kinetic theory of heat}},
  author={Einstein, A.},
  journal={Ann. Phys.-Leipzig},
  volume={31},
  pages={132},
  year={1905}
}

@article{sutherland1905lxxv,
  title={{LXXV. A dynamical theory of diffusion for non-electrolytes and the molecular mass of albumin}},
  author={Sutherland, W.},
  journal={The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science},
  volume={9},
  pages={781--785},
  year={1905},
  publisher={Taylor \& Francis}
}

@article{smoluchowski1906zusammenfassende,
  title={{ZUSAMMENFASSENDE BEARBEITUNGEN.}},
  author={Smoluchowski, Von M v and im unbegrenzten Raum, I Diffusion},
  journal={Ann. Phys.},
  volume={21},
  pages={756},
  year={1906}
}

@article{langevin1908cr,
  title={{CR Acad. Sci.(Paris) 146, 530; trans. Lemons, DS \& Gythiel, A.(1997)}},
  author={Langevin, P.},
  journal={Am. J. Phys},
  volume={65},
  pages={1079--1081},
  year={1908}
}

@article{perrin1908agitation,
  title={{L’agitation mol{\'e}culaire et le mouvement brownien}},
  author={Perrin, J.},
  journal={C. R. Hebd. Acad. Sci.},
  volume={146},
  pages={967--970},
  year={1908}
}

@article{perrin1909movement,
  title={{Movement brownien et realite molec}},
  author={Perrin, J.},
  journal={Ann. Chim. Phys.},
  volume={18},
  pages={1--114},
  year={1909}
}

%%%%% JHUTDB

@misc{jhtdb,
        Author = {{THE TURBULENCE DATABASE GROUP}},
        Title  = "\emph{Johns Hopkins Turbulence Databases}",
        Note   = "\url{http://turbulence.pha.jhu.edu}   [Accessed: February 24th, 2020]",
        year = {2019},
    }

%%%%% OBERLACK LIE SYMMETRIES

@article{grebenev2007approximate,
  title={{Approximate Lie symmetries of the Navier-Stokes equations}},
  author={Grebenev, V. N. and Oberlack, M.},
  journal={J. Nonlinear Math. Phys.},
  volume={14},
  pages={157--163},
  year={2007},
  publisher={Taylor \& Francis}
}

%%%%% THMT'18 CATALOG

  @book{thmt18,
    title={{Exposi{\c{c}}{\~a}o Turbul{\^e}ncia e Arte}},
    author={Guimar{\~a}es, H.},
    year={2018},
    publisher={UFRJ}
  }

%%%%% DISPERSION

@article{boffetta2002,
  title={{Relative dispersion in fully developed turbulence: the Richardson’s law and intermittency corrections}},
  author={Boffetta, G. and Sokolov, I. M.},
  journal={Phys. Rev. Lett.},
  volume={88},
  pages={094501},
  year={2002},
  publisher={APS}
}

@article{salazar2009,
  title={{Two-particle dispersion in isotropic turbulent flows}},
  author={Salazar, J. P. L. C. and Collins, L. R.},
  journal={Annu. Rev. Fluid Mech.},
  volume={41},
  pages={405--432},
  year={2009},
  publisher={Annual Reviews}
}

@article{bourgoin2006,
  title={{The role of pair dispersion in turbulent flow}},
  author={Bourgoin, M. and Ouellette, N. T. and Xu, H. and Berg, J. and Bodenschatz, E.},
  journal={Science},
  volume={311},
  pages={835--838},
  year={2006},
  publisher={American Association for the Advancement of Science}
}

%%%%% RG AND COARSE GRAINING

  @article{hou2001,
    title={{Renormalization group and perfect operators for stochastic differential equations}},
    author={Hou, Q. and Goldenfeld, N. and McKane, A.},
    journal={Phys. Rev. E},
    volume={63},
    pages={036125},
    year={2001},
    publisher={APS}
  }

  @article{goldenfeld1998,
    title={{Block spins for partial differential equations}},
    author={Goldenfeld, N. and McKane, A. and Hou, Q.},
    journal={J. Stat. Phys.},
    volume={93},
    pages={699--714},
    year={1998},
    publisher={Springer}
  }

  @article{chorin2002,
    title={{Optimal prediction with memory}},
    author={Chorin, A. J. and Hald, O. H. and Kupferman, R.},
    journal={Physica D},
    volume={166},
    pages={239--257},
    year={2002},
    publisher={Elsevier}
  }

  @article{chorin1999,
    title={{Unresolved computation and optimal predictions}},
    author={Chorin, A. J. and Kast, A. P. and Kupferman, R.},
    journal={Commun. Pur. Appl. Math.},
    volume={52},
    pages={1231--1254},
    year={1999},
    publisher={Wiley Online Library}
  }

  @article{chorin1998,
    title={{Optimal prediction of underresolved dynamics}},
    author={Chorin, A. J. and Kast, A. P. and Kupferman, R.},
    journal={P. Natl. Acad. Sci. USA},
    volume={95},
    pages={4094--4098},
    year={1998},
    publisher={National Acad Sciences}
  }

%%%%% RODRIGO THESIS

  @phdthesis{pereira2012,
    title={{Cascata log-poissoniana,flutua{\c{c}}{\~o}es de vorticidade e representa{\c{c}}{\~a}o de wavelets em turbul{\^e}ncia homog{\^e}nea}},
    author={Pereira, R. M.},
    year={2012},
    school={Universidade Federal do Rio de Janeiro}
  }

%%%%% INSTANTONS

  @article{schafer1998,
    title={{Instantons in QCD}},
    author={Sch{\"a}fer, T. and Shuryak, E. V.},
    journal={Rev. Mod. Phys.},
    volume={70},
    pages={323},
    year={1998},
    publisher={APS}
  }

@article{orszag1972,
  title={{Numerical simulation of three-dimensional homogeneous isotropic turbulence}},
  author={Orszag, S. A. and Patterson, G. S.},
  journal={Phys. Rev. Lett.},
  volume={28},
  pages={76},
  year={1972},
  publisher={APS}
}

@article{li2008,
  title={{A public turbulence database cluster and applications to study Lagrangian evolution of velocity increments in turbulence}},
  author={Li, Y. and Perlman, E. and Wan, M. and Yang, Y. and Meneveau, C. and Burns, R. and Chen, S. and Szalay, A. and Eyink, G.},
  journal={J. Turbul.},
  pages={N31},
  year={2008},
  publisher={Taylor \& Francis}
}


@book{schlichting2016,
  title={{Boundary-layer theory}},
  author={Schlichting, H. and Gersten, K.},
  year={2016},
  publisher={Springer}
}


@article{feynman1972,
  title={{Statistical Mechanics, A set of lectures}},
  author={Feynman, R. P.},
  journal={Frontiers in Physics. Perseus Books},
  year={1972}
}


  @article{eckert2017,
    title={{A kind of boundary-layer \enquote{flutter}: The turbulent history of a fluid mechanical instability}},
    author={Eckert, M.},
    journal={arXiv preprint arXiv:1706.00334},
    year={2017}
  }

  @article{lin1945,
    title={{On the stability of two-dimensional parallel flows. I. General theory}},
    author={Lin, C.-C.},
    journal={Q. Appl. Math.},
    volume={3},
    pages={117--142},
    year={1945}
  }

  @article{wiener1930generalized,
    title={{Generalized harmonic analysis}},
    author={Wiener, N.},
    journal={Acta Math.},
    volume={55},
    pages={117--258},
    year={1930},
    publisher={Institut Mittag-Leffler}
  }

  @article{taylor1935statistical,
    title={{Statistical theory of turbulence}},
    author={Taylor, G. I.},
    journal={Proc. R. Soc. Lon. Ser.-A},
    volume={151},
    pages={465--478},
    year={1935},
    publisher={The Royal Society}
  }

@article{benzi1993random,
  title={{A random process for the construction of multiaffine fields}},
  author={Benzi, R. and Biferale, L. and Crisanti, A. and Paladin, G. and Vergassola, M. and Vulpiani, A.},
  journal={Physica D},
  volume={65},
  pages={352--358},
  year={1993},
  publisher={Elsevier}
}

@inproceedings{kolmogorov1961precision,
    title={{Pr{\'e}cision sur la structure locale de la turbulence dans un fluide visqueux aux nombres de Reynolds {\'e}l{\'e}v{\'e}s}},
    author={Kolmogorov, A. N.},
    booktitle={M{\'e}canique de la Turbulence},
    year={1961},
    booktitleaddon = {Colloq. Internat. Marseille},
    published = {CNRS, Paris}
  }

@article{kolmogorov1962refinement,
  title={{A refinement of previous hypotheses concerning the local structure of turbulence in a viscous incompressible fluid at high Reynolds number}},
  author={Kolmogorov, A. N.},
  journal={J. Fluid Mech.},
  volume={13},
  pages={82--85},
  year={1962},
  publisher={Cambridge University Press}
}

@article{obukhov1962,
  title={{Some specific features of atmospheric turbulence}},
  author={Obukhov, A. M.},
  journal={J. Fluid Mech.},
  volume={13},
  pages={77--81},
  year={1962},
}

@article{reynolds1883,
  title={{XXIX. An experimental investigation of the circumstances which determine whether the motion of water shall be direct or sinuous, and of the law of resistance in parallel channels}},
  author={Reynolds, O.},
  journal={Philos. T. R. Soc. Lond.},
  pages={935--982},
  year={1883},
  publisher={The Royal Society London}
}

@article{duchon2000,
  title={{Inertial energy dissipation for weak solutions of incompressible Euler and Navier-Stokes equations}},
  author={Duchon, J. and Robert, R.},
  journal={Nonlinearity},
  volume={13},
  pages={249},
  year={2000},
  publisher={IOP Publishing}
}

@misc{tao2019onsager,
    Author = {Tao, T.},
    Title  = {{255B, Notes 2: Onsager’s conjecture}},
    Note   = "\url{https://terrytao.wordpress.com/2019/01/08/255b-notes-2-onsagers-conjecture/} [Accessed: February 24th, 2020]",
    year = 2019,
  }

@article{delellis2012,
  title={{Dissipative Euler flows and Onsager's conjecture}},
  author={De Lellis, C. and Sz{\'e}kelyhidi, L.},
  journal={arXiv preprint arXiv:1205.3626},
  year={2012}
}

@article{constantin1994,
  title={{Onsager's conjecture on the energy conservation for solutions of Euler's equation}},
  author={Constantin, P. and E, W. and Titi, E. S.},
  journal={Commun. Math. Phys.},
  volume={165},
  pages={207--209},
  year={1994},
  publisher={Springer}
}

@article{scheffer1993,
  title={{An inviscid flow with compact support in space-time}},
  author={Scheffer, V.},
  journal={J. Geom. Anal.},
  volume={3},
  pages={343--401},
  year={1993},
  publisher={Springer}
}

@article{shnirelman1997,
  title={{On the nonuniqueness of weak solution of the Euler equation}},
  author={Shnirelman, A.},
  journal={Commun. Pur. Appl. Math.},
  volume={50},
  pages={1261--1286},
  year={1997},
  publisher={Wiley Online Library}
}

@article{delellis2007,
  title={{The Euler equations as a differential inclusion}},
  author={De Lellis, C. and Sz{\'e}kelyhidi, L.},
  journal={arXiv preprint math/0702079},
  year={2007}
}

@article{isett2018,
  title={{A proof of Onsager's conjecture}},
  author={Isett, P.},
  journal={Ann. Math.},
  volume={188},
  pages={871--963},
  year={2018},
  publisher={JSTOR}
}

@article{delellis2019,
  title={{On turbulence and geometry: from Nash to Onsager}},
  author={De Lellis, C. and Sz{\'e}kelyhidi, L.},
  journal={arXiv preprint arXiv:1901.02318},
  year={2019}
}

@article{leray1934,
  title={{Sur le mouvement d'un liquide visqueux emplissant l'espace}},
  author={Leray, J.},
  journal={Acta Math.},
  volume={63},
  pages={193--248},
  year={1934},
  publisher={Institut Mittag-Leffler}
}

@article{hopf1950uber,
  title={{{\"U}ber die Anfangswertaufgabe f{\"u}r die hydrodynamischen Grundgleichungen. Erhard Schmidt zu seinem 75. Geburtstag gewidmet}},
  author={Hopf, E.},
  journal={Math. Nachr.},
  volume={4},
  pages={213--231},
  year={1950},
  publisher={Wiley Online Library}
}

@article{eyink2006,
  title={{Onsager and the theory of hydrodynamic turbulence}},
  author={Eyink, G. L. and Sreenivasan, K. R.},
  journal={Rev. Mod. Phys.},
  volume={78},
  pages={87},
  year={2006},
  publisher={APS}
}


@article{volino2001measurements,
  title={{Measurements in separated and transitional boundary layers under low-pressure turbine airfoil conditions}},
  author={Volino, R. J. and Hultgren, L. S.},
  journal={J. Turbomach.},
  volume={123},
  pages={189--197},
  year={2001},
  publisher={American Society of Mechanical Engineers Digital Collection}
}

@article{van1996modification,
  title={{{Modification of the boundary layer calculation in RFOIL for improved airfoil stall prediction}}},
  author={Van Rooij, R.},
  journal={Report IW-96087R TU-Delft, the Netherlands},
  year={1996}
}

  @book{mussardo2010,
    title={Statistical field theory: An introduction to exactly solved models in statistical physics},
    author={Mussardo, G.},
    year={2010},
    publisher={Oxford University Press}
  }

  @book{amit2005,
    title={{Field theory, the renormalization group, and critical phenomena: Graphs to computers}},
    author={Amit, D. J. and Martin-Mayor, V.},
    year={2005},
    publisher={World Scientific Publishing Company}
  }

  @book{francesco2012,
    title={Conformal field theory},
    author={Francesco, P. and Mathieu, P. and S{\'e}n{\'e}chal, D.},
    year={2012},
    publisher={Springer Science \& Business Media}
  }

%%%%% INSTANTONS HISTORY

@article{gurarie1996,
  title={{Instantons in the Burgers equation}},
  author={Gurarie, V. and Migdal, A.},
  journal={Phys. Rev. E},
  volume={54},
  pages={4908},
  year={1996},
  publisher={APS}
}


@article{balkovsky1997,
  title={{Intermittency of Burgers' turbulence}},
  author={Balkovsky, E. and Falkovich, G. and Kolokolov, I. and Lebedev, V.},
  journal={Phys. Rev. Lett.},
  volume={78},
  pages={1452},
  year={1997},
  publisher={APS}
}

@article{shraiman1994,
  title={{Lagrangian path integrals and fluctuations in random flow}},
  author={Shraiman, B. I. and Siggia, E. D.},
  journal={Phys. Rev. E},
  volume={49},
  pages={2912},
  year={1994},
  publisher={APS}
}

@article{falkovich1996,
  title={Instantons and intermittency},
  author={Falkovich, G. and Kolokolov, I. and Lebedev, V. and Migdal, A.},
  journal={Phys. Rev. E},
  volume={54},
  pages={4896},
  year={1996},
  publisher={APS}
}

@article{polyakov1995,
  title={Turbulence without pressure},
  author={Polyakov, A. M.},
  journal={Phys. Rev. E},
  volume={52},
  pages={6183},
  year={1995},
  publisher={APS}
}

@article{feigelman1980,
  title={One-dimensional periodic structure in a weak random potential},
  author={Feigel'Man, M. V.},
  journal={Soviet Journal of Experimental and Theoretical Physics},
  volume={52},
  pages={555},
  year={1980}
}

@article{cole1951,
  title={On a quasilinear parabolic equation occuring in aerodynamics},
  author={Cole, J. D.},
  journal={Quart. Appl. Math.},
  volume={9},
  pages={225-236},
  year={1951}
  }

@article{hopf1950,
  title={{The partial differential equation $u_t + u u_x = \mu u_{xx}$}},
  author={Hopf, E.},
  journal={Commun. Pur. Appl. Math.},
  volume={3},
  pages={201-230},
  year={1950}
  }

@article{bec2007,
  title={Burgers turbulence},
  author={Bec, J. and Khanin, K.},
  journal={Phys. Rep.},
  volume={447},
  pages={1-66},
  year={2007},
  publisher={Elsevier}
}

@article{chertkov1997,
  title={Instanton for random advection},
  author={Chertkov, M.},
  journal={Phys. Rev. E},
  volume={55},
  pages={2722},
  year={1997},
  publisher={APS}
}

@article{hayn1991,
  title={Instanton approach to the conductivity of a disordered solid},
  author={Hayn, R. and John, W.},
  journal={Nucl. Phys. B},
  volume={348},
  pages={766-786},
  year={1991},
  publisher={Elsevier}
}

@book{ellis2007,
  title={Entropy, large deviations, and statistical mechanics},
  author={Ellis, R. S.},
  year={2007},
  publisher={Springer}
}

@article{touchette2009,
  title={The large deviation approach to statistical mechanics},
  author={Touchette, H.},
  journal={Phys. Rep.},
  volume={478},
  pages={1-69},
  year={2009},
  publisher={Elsevier}
}

%%%%% BOOKS

@book{gardiner2009,
  title={Stochastic methods},
  author={Gardiner, C.},
  year={2009},
  published={Springer Berlin}
  }

@article{ito1944,
  title={Stochastic integral},
  author={It{\^o}, K.},
  journal={Proc. Imp. Acad. Jpn.},
  volume={20},
  pages={519--524},
  year={1944},
  publisher={The Japan Academy}
}

@inproceedings{bachelier1900,
  title={Th{\'e}orie de la sp{\'e}culation},
  author={Bachelier, L.},
  booktitle={Annales scientifiques de l'{\'E}cole normale sup{\'e}rieure},
  volume={17},
  pages={21--86},
  year={1900}
}

@book{vankampen1992,
  title={Stochastic processes in physics and chemistry},
  author={Van Kampen, N. G.},
  year={1992},
  publisher={Elsevier}
}

@article{mori1975,
  title={Stochastic processes of macroscopic variables},
  author={Mori, H.},
  journal={Prog. Theor. Phys.},
  volume={53},
  pages={1617},
  year={1975}
}

@book{protter2005,
  title={Stochastic differential equations},
  author={Protter, P.},
  year={2005},
  publisher={Springer}
}

@book{evans2012,
  title={An introduction to stochastic differential equations},
  author={Evans, L. C.},
  volume={82},
  year={2012},
  publisher={American Mathematical Soc.}
}

@article{vankampen1981,
  title={{It{\^o} versus Stratonovich}},
  author={Van Kampen, N. G.},
  journal={Journal of Statistical Physics},
  volume={24},
  pages={175--187},
  year={1981},
  publisher={Springer}
}

@article{mannella2012,
  title={It{\^o} versus Stratonovich: 30 years later},
  author={Mannella, R. and McClintock, P. V. E.},
  journal={Fluctuation and Noise Letters},
  volume={11},
  pages={1240010},
  year={2012},
  publisher={World Scientific}
}

%%%%% RFD references

@article{moriconi2014,
  title={{Velocity-gradient probability distribution functions in a Lagrangian model of turbulence}},
  author={Moriconi, L. and Pereira, R. M. and Grigorio, L. S.},
  journal={J. Stat. Mech.},
  volume={2014},
  pages={P10015},
  year={2014},
  publisher={IOP Publishing}
}

@article{johnson2016closure,
  title={A closure for Lagrangian velocity gradient evolution in turbulence using recent-deformation mapping of initially Gaussian fields},
  author={Johnson, P. L. and Meneveau, C.},
  journal={J. Fluid Mech.},
  volume={804},
  pages={387--419},
  year={2016},
  publisher={Cambridge University Press}
}

@book{Barabasi,
  title={Fractal concepts in surface growth},
  author={Barab{\'a}si, A.-L. and Stanley, H. E.},
  year={1995},
  publisher={Cambridge university press}
}

@article{chevillard2006,
  title = {Lagrangian dynamics and statistical geometric structure of turbulence},
  author = {Chevillard, L. and Meneveau, C.},
  journal = {Phys. Rev. Lett.},
  volume = {97},
  issue = {17},
  pages = {174501},
  year = {2006},
}

@article{pereira2018multifractal,
  title={A multifractal model for the velocity gradient dynamics in turbulent flows},
  author={Pereira, R. M. and Moriconi, L. and Chevillard, L.},
  journal={J. Fluid Mech.},
  volume={839},
  pages={430--467},
  year={2018},
  publisher={Cambridge University Press}
}

@article{chevillardetal2006,
author = {L. Chevillard and B. Castaing and E. Lévêque and A. Arneodo},
title = {Unified multifractal description of velocity increments statistics in turbulence: Intermittency and skewness },
journal = {Physica D},
volume = {218},
pages = {77},
year = {2006},
}


@article{kogut1979introduction,
  title={An introduction to lattice gauge theory and spin systems},
  author={Kogut, J. B.},
  journal={Rev. Mod. Phys.},
  volume={51},
  pages={659},
  year={1979},
  publisher={APS}
}

@book{feynman2010quantum,
  title={Quantum Mechanics and path integrals},
  author={Feynman, R. P. and Hibbs, A. R. and Styer, D. F.},
  year={2010},
  publisher={Courier Corporation}
}

@book{Peskin,
  title={An Introduction to Quantum Field Theory},
  author={Peskin, M. E. and Schroeder, D. V.},
  year=1995,
  publisher={Addison-Wesley Publishing Company}
}

@article{tsinober1992experimental,
  title={Experimental investigation of the field of velocity gradients in turbulent flows},
  author={Tsinober, A. and Kit, E. and Dracos, T.},
  journal={J. Fluid Mech.},
  volume={242},
  pages={169--192},
  year={1992},
  publisher={Cambridge University Press}
}

@article{she1994universal,
  title={Universal scaling laws in fully developed turbulence},
  author={She, Z.-S. and Leveque, E.},
  journal={Phys. Rev. Lett.},
  volume={72},
  pages={336},
  year={1994},
  publisher={APS}
}

@article{dubrulle1994intermittency,
  title={Intermittency in fully developed turbulence: Log-Poisson statistics and generalized scale covariance},
  author={Dubrulle, B.},
  journal={Phys. Rev. Lett.},
  volume={73},
  pages={959},
  year={1994},
  publisher={APS}
}

@article{girimaji90material,
  title={Material-element deformation in isotropic turbulence},
  author={Girimaji, S. S. and Pope, S. B.},
  journal={J. Fluid Mech.},
  volume={220},
  pages={427--458},
  year={1990},
  publisher={Cambridge University Press}
}

@article{chernykh2001,
  title={Large negative velocity gradients in Burgers turbulence},
  author={Chernykh, A. I. and Stepanov, M. G.},
  journal={Phys. Rev. E},
  volume={64},
  pages={026306},
  year={2001},
  publisher={APS}
}

@article{moriconi2004,
  title={Statistics of intense turbulent vorticity events},
  author={Moriconi, L.},
  journal={Phys. Rev. E},
  volume={70},
  pages={025302},
  year={2004},
  publisher={APS}
}

@article{falkovich2011,
  title={Vorticity statistics in the direct cascade of two-dimensional turbulence},
  author={Falkovich, G. and Lebedev, V.},
  journal={Phys. Rev. E},
  volume={83},
  pages={045301},
  year={2011},
  publisher={APS}
}

@article{grigorio2017instantons,
  title={Instantons in a Lagrangian model of turbulence},
  author={Grigorio, L. S. and Bouchet, F. and Pereira, R. M. and Chevillard, L.},
  journal={J. Phys. A},
  volume={50},
  pages={055501},
  year={2017},
  publisher={IOP Publishing}
}

@article{afonso2010recent,
  title={Recent fluid deformation closure for velocity gradient tensor dynamics in turbulence: Timescale effects and expansions},
  author={Afonso, M. M. and Meneveau, C.},
  journal={Physica D},
  volume={239},
  pages={1241--1250},
  year={2010},
  publisher={Elsevier}
}

@book{tsinober2009,
  title={An Informal Conceptual Introduction to Turbulence},
  author={A. Tsinober},
  year={2009},
  publisher={Springer Netherlands}
}

@article{moriconi2013,
  title = {Vorticity statistics and the time scales of turbulent strain},
  author = {Moriconi, L.  and Pereira, R. M.},
  journal = {Phys. Rev. E},
  volume = {88},
  issue = {1},
  pages = {013005},
  year = {2013}
  }

@article{kholmyansky2009,
  title = {Log-Poisson cascade description of turbulent velocity-gradient statistics},
  author = {Kholmyansky, M. and Moriconi, L. and Pereira, R. M. and Tsinober, A.},
  journal = {Phys. Rev. E},
  volume = {80},
  pages = {036311},
  year = {2009}
}

@article{batchelor1949,
  title={The nature of turbulent motion at large wave-numbers},
  author={Batchelor, G. K. and Townsend, A. A.},
  journal={P. Roy. Soc. Lond. A Mat.},
  volume={199},
  pages={238--255},
  year={1949}
}

@phdthesis{leorat1975,
  title={La turbulence magn{\'e}tohydrodynamique h{\'e}licitaire et la g{\'e}n{\'e}ration des champs magn{\'e}tiques a grande {\'e}chelle},
  author={Leorat, J.},
  school={Univ.Paris VII},
  year={1975}
}

@article{vieillefosse1982,
  title={Local interaction between vorticity and shear in a perfect incompressible fluid},
  author={Vieillefosse, P.},
  journal={J. Physique},
  volume={43},
  pages={837--842},
  year={1982},
  publisher={Soci{\'e}t{\'e} Fran{\c{c}}aise de Physique}
}

@article{vieillefosse1984,
  title={Internal motion of a small element of fluid in an inviscid flow},
  author={Vieillefosse, P.},
  journal={Physica A},
  volume={125},
  pages={150--162},
  year={1984},
  publisher={Elsevier}
}

@article{chevillard2008modeling,
  title={Modeling the pressure Hessian and viscous Laplacian in turbulence: comparisons with direct numerical simulation and implications on velocity gradient dynamics},
  author={Chevillard, L. and Meneveau, C. and Biferale, L. and Toschi, F.},
  journal={Phys. Fluids},
  volume={20},
  pages={101504},
  year={2008},
  publisher={AIP}
}

@book{pope2000,
  title={Turbulent flows},
  author={Pope, S. B.},
  year={2001},
  publisher={IOP Publishing}
}

%%%%% SADDLE POINT IN DISORDERED SYSTEMS

@article{zittartz1966,
  title={Theory of bound states in a random potential},
  author={Zittartz, J. and Langer, J. S.},
  journal={Phys. Rev.},
  volume={148},
  pages={741},
  year={1966},
  publisher={APS}
}

@article{langer1967,
  title={Theory of the condensation point},
  author={Langer, J. S.},
  journal={Ann. Physics},
  volume={41},
  pages={108-57},
  year={1967}
}

@article{langer1969,
  title={Statistical theory of the decay of metastable states},
  author={Langer, J. S.},
  journal={Ann. Phys.},
  volume={54},
  pages={258--275},
  year={1969}
}


@article{belavin1975,
  title={{Pseudoparticle solutions of the Yang-Mills equations}},
  author={Belavin, A. A. and Polyakov, A. M. and Schwartz, A. S. and Tyupkin, Y. S.},
  journal={Phys. Lett. B},
  volume={59},
  pages={85--87},
  year={1975}
}

@misc{canet2019leshouches,
  author        = {Canet, L.},
  title         = {Time dependence of correlation functions in homogeneous and isotropic turbulence},
  year          = {2019},
  institution = {Ecole de Physique des Houches},
  howpublished = {Lecture notes},
  note   = "\url{http://www.nctr.eu/images/2019/lectures/Lecture_Canet_NCTRV.pdf} [Accessed: February 24th, 2020]",
}

@misc{perrinAIP,
    Author = {{AMERICAN INSTITUTE OF PHYSICS}},
    Title  = {{Jean Perrin}},
    Note   = "\url{https://history.aip.org/phn/11807006.html} [Accessed: February 24th, 2020]",
    year = {2019},
  }

@article{forster1977,
  title={Large-distance and long-time properties of a randomly stirred fluid},
  author={Forster, D. and Nelson, D. R. and Stephen, M. J.},
  journal={Phys. Rev. A},
  volume={16},
  pages={732},
  year={1977},
  publisher={APS}
}


@article{varadhan1966,
  title={Asymptotic probabilities and differential equations},
  author={Varadhan, S. R. S.},
  journal={Commun. Pur. Appl. Math.},
  volume={19},
  pages={261--286},
  year={1966},
  publisher={Wiley Online Library}
}

@book{canuto2012spectral,
  title={Spectral methods in fluid dynamics},
  author={Canuto, C. and Hussaini, M. Y. and Quarteroni, A. and Thomas Jr, A.},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@book{Kardar,
  title={Statistical physics of fields},
  author={Kardar, M.},
  year={2007},
  publisher={Cambridge University Press}
}

@article{ChevPRL,
  title = {Lagrangian dynamics and statistical geometric structure of turbulence},
  author = {Chevillard, L. and Meneveau, C.},
  journal = {Phys. Rev. Lett.},
  volume = {97},
  issue = {17},
  pages = {174501},
  numpages = {4},
  year = {2006},
}

@book{frisch1995,
  title={{Turbulence: The legacy of A. N. Kolmogorov}},
  author={U. Frisch},
  year={1995},
  publisher={Cambridge University Press}
}

@article{Chev2006,
author = {Chevillard, L. and Castaing, B. and Lévêque, E. and Arneodo, A.},
title = {Unified multifractal description of velocity increments statistics in turbulence: Intermittency and skewness },
journal = {Physica D},
volume = {218},
pages = {77},
year = {2006},
}

@book{zinn2002,
  title={Quantum Field Theory and Critical Phenomena},
  author={Zinn-Justin, J.},
  year=2002,
  publisher={Clarendon Press}
}



@article{Girimaji90,
  title={Material-element deformation in isotropic turbulence},
  author={Girimaji, SS and Pope, SB},
  journal={J. Fluid Mech.},
  volume={220},
  pages={427--458},
  year={1990},
  publisher={Cambridge University Press}
}

@article{Wallace9,
  title={The velocity and vorticity vector fields of a turbulent boundary layer},
  author={Vukoslavcevic, P. and Wallace, J. and Balint, J. L.},
  journal={J. Fluid Mech.},
  volume={228},
  pages={25},
  year={1991},
}

@article{grafke2015relevance,
  title={Relevance of instantons in Burgers turbulence},
  author={Grafke, T. and Grauer, R. and Sch{\"a}fer, T. and Vanden-Eijnden, E.},
  journal={Europhys. Lett.},
  volume={109},
  pages={34003},
  year={2015},
  publisher={IOP Publishing}
}

@article{grafke2015instanton,
  title={The instanton method and its numerical implementation in fluid mechanics},
  author={Grafke, T. and Grauer, R. and Sch{\"a}fer, T.},
  journal={J. Phys. A},
  volume={48},
  pages={333001},
  year={2015},
  publisher={IOP Publishing}
}

@article{MoriconiPereiraKholmyansky,
  title = {Log-Poisson cascade description of turbulent velocity-gradient statistics},
  author = {Kholmyansky, M. and Moriconi, L. and Pereira, R. M. and Tsinober, A.},
  journal = {Phys. Rev. E},
  volume = {80},
  pages = {036311},
  year = {2009}
}

@article{BatchelorTownsend1949,
  title={The nature of turbulent motion at large wave-numbers},
  author={Batchelor, G. K. and Townsend, A. A.},
  journal={P. Roy. Soc. Lond. A Mat.},
  volume={199},
  pages={238--255},
  year={1949}
}

@phdthesis{leorat1975turbulence,
  title={La turbulence magn{\'e}tohydrodynamique h{\'e}licitaire et la g{\'e}n{\'e}ration des champs magn{\'e}tiques a grande {\'e}chelle},
  author={Leorat, J.},
  school={Univ.Paris VII},
  year={1975}
}

@book{rajaraman1987,
  title={Solitons and Instantons: An Introduction to Solitons and Instantons in Quantum Field Theory},
  author={Rajaraman, R.},
  year={1987},
  publisher={Elsevier}
}

@article{burgers1948,
  author={Burgers, J. M.},
  title={A mathematical model illustrating the theory of turbulence},
  journal={Adv. Appl. Mech.},
  volume={1},
  page={171},
  year={1948}
}

@article{vonneumann1963,
  title={Recent theories of turbulence},
  author={von Neumann, J.},
  journal={Collected works (1949-1963)},
  volume={6},
  pages={437--472},
  year={1963},
  publisher={Pergamon Press}
}

@book{gurbatov1991,
  title={Nonlinear random waves and turbulence in nondispersive media: waves, rays, particles},
  author={Gurbatov, S. N. and Malakhov, A. N.},
  year={1991},
  publisher={Manchester University Press}
}

@article{zeldovich1970,
  title={{Gravitational instability: An approximate theory for large density perturbations}},
  author={Zel'Dovich, Ya. B.},
  journal={Astron. Astrophys.},
  volume={5},
  pages={84},
  year={1970}
}

@article{gurbatov1984,
  title={Probability distributions and spectra of potential hydrodynamic turbulence},
  author={Gurbatov, S. N. and Saichev, A. I.},
  journal={Radiofizika},
  volume={27},
  pages={456--468},
  year={1984}
}

@article{kardar1986,
  title={Dynamic scaling of growing interfaces},
  author={Kardar, M. and Parisi, G. and Zhang, Y.-C.},
  journal={Phys. Rev. Lett.},
  volume={56},
  pages={889},
  year={1986},
  publisher={APS}
}

@article{musha1978,
  title={{Traffic current fluctuation and the Burgers equation}},
  author={Musha, T. and Higuchi, H.},
  journal={Japanese journal of applied physics},
  volume={17},
  pages={811},
  year={1978},
  publisher={IOP Publishing}
}

@article{chowdhury2000,
  title={Statistical physics of vehicular traffic and some related systems},
  author={Chowdhury, D. and Santen, L. and Schadschneider, A.},
  journal={Phys. Rep.},
  volume={329},
  pages={199--329},
  year={2000},
  publisher={Elsevier}
}

@book{petrovskii2005,
  title={Exactly solvable models of biological invasion},
  author={Petrovskii, S. V. and Li, B.-L.},
  year={2005},
  publisher={Chapman and Hall/CRC}
}

@article{khanin1997,
  title={{Probability distribution functions for the random forced Burgers equation}},
  author={E, W. and Khanin, K. and Mazel, A. and Sinai, Y.},
  journal={Physical Review Letters},
  volume={78},
  pages={1904},
  year={1997},
  publisher={APS}
}

@article{bec2001,
  title={{Universality of velocity gradients in forced Burgers turbulence}},
  author={Bec, J.},
  journal={Phys. Rev. Lett.},
  volume={87},
  pages={104501},
  year={2001},
  publisher={APS}
}

@article{moriconi2009,
  title={{Instanton theory of Burgers shocks and intermittency}},
  author={Moriconi, L.},
  journal={Phys. Rev. E},
  volume={79},
  pages={046324},
  year={2009},
  publisher={APS}
}

@book{cardy1996,
  title={Scaling and renormalization in statistical physics},
  author={Cardy, J.},
  volume={5},
  year={1996},
  publisher={Cambridge university press}
}

@article{margazoglou2019,
  title={Hybrid monte carlo algorithm for sampling rare events in space-time histories of stochastic fields},
  author={Mar\-ga\-zo\-glou, G. and Bi\-fe\-ra\-le, L. and Gra\-uer, R. and Jan\-sen, K. and Mes\-ter\-h{\'a}\-zy, D. and Ro\-se\-now, T. and Tri\-pi\-cci\-one, R.},
  journal={Phys. Rev. E},
  volume={99},
  pages={053303},
  year={2019},
  publisher={APS}
}

@article{ebener2019,
  title={{Instanton based importance sampling for rare events in stochastic PDEs}},
  author={Ebener, L. and Margazoglou, G. and Friedrich, J. and Biferale, L. and Grauer, R.},
  journal={Chaos},
  volume={29},
  pages={063102},
  year={2019},
  publisher={AIP Publishing}
}

@article{gotoh1998,
  title={{Steady-state Burgers turbulence with large-scale forcing}},
  author={Gotoh, T. and Kraichnan, R. H.},
  journal={Phys. Fluids},
  volume={10},
  pages={2859--2866},
  year={1998},
  publisher={AIP}
}

@book{coleman1988,
  title={Aspects of symmetry},
  author={Coleman, S.},
  year={1988},
  publisher={Cambridge University Press}
}

@book{langouche1982,
  title={Functional integration and semiclassical expansions},
  author={Langouche, F. and Roekaerts, Dirk and Tirapegui, Enrique},
  year={1982},
  publisher={Springer Science \& Business Media}
}


@book{kloeden2013,
  title={Numerical solution of stochastic differential equations},
  author={Kloeden, P. E. and Platen, E.},
  volume={23},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{smith1997,
  title={Onset of intermittency in two-dimensional decaying turbulence},
  author={Smith, L. M. and Yakhot, V.},
  journal={Phys. Rev. E},
  volume={55},
  pages={5458},
  year={1997},
  publisher={APS}
}

@article{forman1987,
  title={Functional determinants and geometry},
  author={Forman, R.},
  journal={Inventiones mathematicae},
  volume={88},
  pages={447--493},
  year={1987},
  publisher={Springer}
}

@article{mckane1995,
  author={McKane, A. J. and Tarlie, J. M. B.},
  journal={J. Phys. A},
  volume={28},
  page={6391},
  year={1995}
  }

@article{muratore2003,
  title={{Path integration over closed loops and Gutzwiller's trace formula}},
  author={Muratore-Ginanneschi, P.},
  journal={Phys. Rep.},
  volume={383},
  pages={299--397},
  year={2003},
  publisher={Elsevier}
}

@article{frisch2005,
  title={Does multifractal theory of turbulence have logarithms in the scaling relations?},
  author={Frisch, U. and Afonso, M. M. and Mazzino, A. and Yakhot, V.},
  journal={J. Fluid Mech.},
  volume={542},
  pages={97--103},
  year={2005},
  publisher={Cambridge University Press}
}

@misc{elgindi2019,
    title={{Finite-time singularity formation for $C^{1,α}$ solutions to the incompressible Euler equations on $\mathbb{R}^3$}},
    author={Elgindi, T. M.},
    year={2019},
    eprint={1904.04795},
    archivePrefix={arXiv},
    primaryClass={math.AP}
}

@misc{elgindighoul2019,
    title={{On the stability of self-similar blow-up for $C^{1,α}$ solutions to the incompressible Euler equations on $\mathbb{R}^3$}},
    author={Elgindi, T. M. and Ghoul, T.-E. and Masmoudi, N.},
    year={2019},
    eprint={1910.14071},
    archivePrefix={arXiv},
    primaryClass={math.AP}
}

@misc{hartnett2019euler,
   title={Famous Fluid Equations Spring a Leak},
   note="\url{https://www.quantamagazine.org/mathematician-makes-euler-equations-blow-up-20191218/}[Accessed: February 24th, 2020]",
   journal={Quanta magazine},
   author={Hartnett, K.},
   year={2019}
   }

% appendix cumulants
@article{cumulants,
  author = {McCullagh, P.  and Kolassa, J. },
  title   = {{C}umulants},
  year    = {2009},
  journal = {Scholarpedia},
  volume  = {4},
  pages   = {4699},
  DOI     = {10.4249/scholarpedia.4699},
  note    = {revision \#137322}
}

@misc{oeis_cumul,
    author = {{OEIS Foundation Inc.}},
    Title  = {A127671},
    Note   = "\url{http://oeis.org/A123456} [Accessed: February 24th, 2020]",
    year = {2019},
  }

@misc{novak2012,
    title={Three lectures on free probability},
    author={Novak, J. and LaCroix, M.},
    year={2012},
    eprint={1205.2097},
    archivePrefix={arXiv},
    primaryClass={math.CO}
}

@article{giardina2006,
  title={Direct evaluation of large-deviation functions},
  author={Giardina, C. and Kurchan, J. and Peliti, L.},
  journal={Phys. Rev. Lett.},
  volume={96},
  number={12},
  pages={120603},
  year={2006},
  publisher={APS}
}

@article{giardina2011,
  title={Simulating rare events in dynamical processes},
  author={Giardina, C. and Kurchan, J. and Lecomte, V. and Tailleur, J.},
  journal={J. Stat. Phys.},
  volume={145},
  pages={787--811},
  year={2011},
  publisher={Springer}
}

@article{perpete2011,
  title={A discrete log-normal process to sequentially generate a multifractal time series},
  author={Perp{\`e}te, N. and Schmitt, F. G.},
  journal={J. Stat. Mech.},
  volume={2011},
  pages={P12013},
  year={2011},
  publisher={IOP Publishing}
}

@article{iyer2019,
  title={{Circulation in high Reynolds number isotropic turbulence is a bifractal}},
  author={Iyer, K. P. and Sreenivasan, K. R. and Yeung, P. K.},
  journal={Phys. Rev. X},
  volume={9},
  pages={041006},
  year={2019},
  publisher={APS}
}

@book{ting2016,
  title={Basics of engineering turbulence},
  author={Ting, D.},
  year={2016},
  publisher={Academic Press}
}

@book{dewan2010,
  title={Tackling turbulent flows in engineering},
  author={Dewan, A.},
  year={2010},
  publisher={Springer Science \& Business Media}
}

@article{tao2016finite,
  title={{Finite time blowup for an averaged three-dimensional Navier-Stokes equation}},
  author={Tao, T.},
  journal={J. Am. Math. Soc.},
  volume={29},
  pages={601--674},
  year={2016}
}

@article{willert1991,
  title={Digital particle image velocimetry},
  author={Willert, C. E. and Gharib, M.},
  journal={Exp. Fluids},
  volume={10},
  pages={181--193},
  year={1991},
  publisher={Springer}
}


@article{adrian2005,
  title={Twenty years of particle image velocimetry},
  author={Adrian, R. J.},
  journal={Exp. Fluids},
  volume={39},
  pages={159--169},
  year={2005},
  publisher={Springer}
}

% limitations and hypotheses of the Navier-Stokes equations
@book{kremer2010,
  title={{An introduction to the Boltzmann equation and transport processes in gases}},
  author={Kremer, G. M.},
  year={2010},
  publisher={Springer Science \& Business Media}
}

@article{mejia2012,
  title={{Nonperturbative renormalization group study of the stochastic Navier-Stokes equation}},
  author={Mej{\'i}a-Mo\-nas\-te\-rio, C. and Mu\-ra\-to\-re-Gi\-nan\-nes\-chi, P.},
  journal={Phys. Rev. E},
  volume={86},
  pages={016315},
  year={2012},
  publisher={APS}
}

@article{furstenberg1963,
  title={The structure of distal flows},
  author={Furstenberg, H.},
  journal={Am. J. Math.},
  volume={85},
  pages={477--515},
  year={1963},
  publisher={JSTOR}
}

@article{zeldovich1984,
  title={Kinematic dynamo problem in a linear velocity field},
  author={Zel'Dovich, Ya. B. and Ruzmaikin, A. A. and Molchanov, S. A. and Sokoloff, D. D.},
  journal={J. Fluid Mech.},
  volume={144},
  pages={1--11},
  year={1984},
  publisher={Cambridge University Press}
}

@article{gawedzki2002,
  title={Soluble models of turbulent advection},
  author={Gawedzki, K.},
  journal={arXiv preprint nlin/0207058},
  year={2002}
}

@article{gawedzki2000,
  title={Phase transition in the passive scalar advection},
  author={Gawedzki, K. and Vergassola, M.},
  journal={Physica D},
  volume={138},
  pages={63--90},
  year={2000},
  publisher={Elsevier}
}

@misc{bernard2000,
  title={Turbulence for (and by) amateurs},
  author={Bernard, D.},
  archivePrefix = {arXiv},
  eprint        = {cond-mat/0007106},
  year = {2020}
}

@misc{perrinnobel,
  Author = {{NOBELPRIZE.ORG}},
  Title  = {Jean Baptiste Perrin - Nobel Lecture},
  Note   = "\url{https://www.nobelprize.org/prizes/physics/1926/perrin/lecture/} [Accessed: February 24th, 2020]",
  year = {2020},
}

@article{frisch1991global,
  title={{From global scaling, a la Kolmogorov, to local multifractal scaling in fully developed turbulence}},
  author={Frisch, U.},
  journal={P. Roy. Soc. Lond. A Mat.},
  volume={434},
  pages={89--99},
  year={1991},
  publisher={The Royal Society London}
}

@article{boffetta2017,
  title={Chaos and predictability of homogeneous-isotropic turbulence},
  author={Boffetta, G. and Musacchio, S.},
  journal={Phys. Rev. Lett.},
  volume={119},
  pages={054102},
  year={2017},
  publisher={APS}
}

@article{berera2018,
  title={Chaotic properties of a turbulent isotropic fluid},
  author={Berera, A. and Ho, R. D. J. G.},
  journal={Phys. Rev. Lett.},
  volume={120},
  pages={024101},
  year={2018},
  publisher={APS}
}

@article{eyink2011,
  title={Stochastic flux freezing and magnetic dynamo},
  author={Eyink, G. L.},
  journal={Phys. Rev. E},
  volume={83},
  pages={056405},
  year={2011},
  publisher={APS}
}

@article{bitane2013,
  title={Geometry and violent events in turbulent pair dispersion},
  author={Bitane, R. and Homann, H. and Bec, J.},
  journal={J. Turbul.},
  volume={14},
  pages={23--45},
  year={2013},
  publisher={Taylor \& Francis}
}

@article{dematteis2018,
  title={Rogue waves and large deviations in deep sea},
  author={Dematteis, G. and Grafke, T. and Vanden-Eijnden, E.},
  journal={P. Natl. Acad. Sci. USA},
  volume={115},
  pages={855--860},
  year={2018},
  publisher={National Acad Sciences}
}

@article{balkovsky1998instanton,
  title={{Instanton for the Kraichnan passive scalar problem}},
  author={Balkovsky, E. and Lebedev, V.},
  journal={Phys. Rev. E},
  volume={58},
  pages={5776},
  year={1998},
  publisher={APS}
}

@article{voth2017,
  title={Anisotropic particles in turbulence},
  author={Voth, G. and Soldati, A.},
  journal={Annu. Rev. Fluid Mech.},
  volume={49},
  pages={249--276},
  year={2017},
  publisher={Annual Reviews}
}

@article{rhodes2014,
  title={Gaussian multiplicative chaos and applications: a review},
  author={Rhodes, R. and Vargas, V.},
  journal={Probability Surveys},
  volume={11},
  year={2014}
}

@article{kahane1985,
  title={{Sur le chaos multiplicatif}},
  author={Kahane, J. P.},
  journal={Ann. Sci. Math. Québec},
  year={1985},
  volume={9},
  page={105}
}

@article{lejan2002,
  title={Integration of brownian vector fields},
  author={Le Jan, Y. and Raimond, O.},
  journal={Ann. Probab.},
  volume={30},
  pages={826--873},
  year={2002},
  publisher={Institute of Mathematical Statistics}
}

@misc{equationsproject,
  Author = {Bobroff, J.},
  Title  = {Physics reimagined},
  Note   = "\url{http://hebergement.u-psud.fr/supraconductivite/equationsnavier_en.html} [Accessed: February 24th, 2020]",
  year = {2012},
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% new bib from shotnoise paper %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@incollection{mandelbrot1972,
  title={{Possible refinement of the lognormal hypothesis concerning the distribution of energy dissipation in intermittent turbulence}},
  author={Mandelbrot, B. B.},
  booktitle={Statistical models and turbulence},
  pages={333--351},
  year={1972},
  publisher={Springer}
}

@article{casella2011,
  title={{Exact simulation of jump-diffusion processes with Monte Carlo applications}},
  author={Casella, B. and Roberts, G. O.},
  journal={Methodol. Comput. Appl.},
  volume={13},
  pages={449--473},
  year={2011},
  publisher={Springer}
}

@book{klebaner2012,
  title={{Introduction to stochastic calculus with applications}},
  author={Klebaner, F. C.},
  year={2012},
  publisher={World Scientific Publishing Company}
}

@article{giesecke2013,
  title={{Exact sampling of jump diffusions}},
  author={Giesecke, K. and Smelov, D.},
  journal={Operations Research},
  volume={61},
  pages={894--907},
  year={2013},
  publisher={INFORMS}
}

@article{giesecke2011,
  title={{Exact simulation of point processes with stochastic intensities}},
  author={Giesecke, K. and Kakavand, H. and Mousavi, M.},
  journal={Oper. Res.},
  volume={59},
  pages={1233--1245},
  year={2011},
  publisher={INFORMS}
}

@article{pollock2016,
  title={On the exact and $\backslash\varepsilon$-strong simulation of (jump) diffusions},
  author={Pollock, M. and Johansen, A. M. and Roberts, G. O.},
  journal={Bernoulli},
  volume={22},
  pages={794--856},
  year={2016},
  publisher={Bernoulli Society for Mathematical Statistics and Probability}
}

@article{gonccalves2014,
  title={{Exact simulation problems for jump-diffusions}},
  author={Gon{\c{c}}alves, F. B. and Roberts, G. O.},
  journal={Methodol. Comput. Appl.},
  volume={16},
  pages={907--930},
  year={2014},
  publisher={Springer}
}

%%%%% Review on Lagrangian Statistics
@article{toschi2009,
  title={{Lagrangian properties of particles in turbulence}},
  author={Toschi, F. and Bodenschatz, E.},
  journal={Annu. Rev. Fluid Mech.},
  volume={41},
  pages={375--404},
  year={2009},
  publisher={Annual Reviews}
}

@article{berestycki2017,
  title={{An elementary approach to Gaussian multiplicative chaos}},
  author={Berestycki, N.},
  journal={Electron. Commun. Prob.},
  volume={22},
  year={2017},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}

@article{schmitt2003,
  title={{A causal multifractal stochastic equation and its statistical properties}},
  author={Schmitt, F. G.},
  journal={Eur. Phys. J. B},
  volume={34},
  pages={85--98},
  year={2003},
  publisher={Springer}
}

@article{girimaji1990diffusion,
  title={{A diffusion model for velocity gradients in turbulence}},
  author={Girimaji, S. S. and Pope, S. B.},
  journal={Phys. Fluids A},
  volume={2},
  pages={242--256},
  year={1990},
  publisher={AIP}
}

@article{iyer2017,
  title={{Reynolds number scaling of velocity increments in isotropic turbulence}},
  author={Iyer, K. P. and Sreenivasan, K. R. and Yeung, P. K.},
  journal={Phys. Rev. E},
  volume={95},
  pages={021101},
  year={2017},
  publisher={APS}
}

@article{robert2010,
  title={{Gaussian multiplicative chaos revisited}},
  author={Robert, R. and Vargas, V.},
  journal={Ann. Probab.},
  volume={38},
  pages={605--631},
  year={2010},
  publisher={Institute of Mathematical Statistics}
}
% here they propose to make rigorous sense of the
% Mandelbrot limit-lognormal model

@article{drivas2019,
  title={{Turbulent cascade direction and Lagrangian time-asymmetry}},
  author={Drivas, T. D.},
  journal={J. Nonlinear Sci.},
  volume={29},
  year={2019},
  publisher={Springer}
}

@article{chevillard2017,
  title={{Regularized fractional Ornstein-Uhlenbeck processes and their relevance to the modeling of fluid turbulence}},
  author={Chevillard, L.},
  journal={Phys. Rev. E},
  volume={96},
  pages={033111},
  year={2017},
  publisher={APS}
}

@article{das2019,
  title={{On the Reynolds number dependence of velocity-gradient structure and dynamics}},
  author={Das, R. and Girimaji, S. S.},
  journal={J. Fluid Mech.},
  volume={861},
  pages={163--179},
  year={2019},
  publisher={Cambridge University Press}
}

@article{watteaux2019,
  title={{On the time scales and structure of Lagrangian intermittency in homogeneous isotropic turbulence}},
  author={Watteaux, R. and Sardina, G. and Brandt, L. and Iudicone, D.},
  journal={J. Fluid Mech.},
  volume={867},
  pages={438--481},
  year={2019},
  publisher={Cambridge University Press}
}

@article{schertzer1997,
  title={{Multifractal cascade dynamics and turbulent intermittency}},
  author={Schertzer, D. and Lovejoy, S. and Schmitt, F. G. and Chigirinskaya, Y. and Marsan, D.},
  journal={Fractals},
  volume={5},
  pages={427--471},
  year={1997},
  publisher={World Scientific}
}

@article{bacry2003,
  title={{Log-infinitely divisible multifractal processes}},
  author={Bacry, E. and Muzy, J.-F.},
  journal={Commun. Math. Phys.},
  volume={236},
  pages={449--475},
  year={2003},
  publisher={Springer}
}

@article{nguyen2019,
  title={Local estimates of H{\"o}lder exponents in turbulent vector fields},
  author={Nguyen, F. and Laval, J.-P. and Kestener, P. and Cheskidov, A. and Shvydkoy, R. and Dubrulle, B.},
  journal={Physical Review E},
  year={2019}
}

@article{johnson2016,
  title={{A closure for Lagrangian velocity gradient evolution in turbulence using recent-deformation mapping of initially Gaussian fields}},
  author={Johnson, P. L. and Meneveau, C.},
  journal={J. Fluid Mech.},
  volume={804},
  pages={387--419},
  year={2016},
  publisher={Cambridge University Press}
}

@article{wallace2010,
  title={{Measurement of the velocity gradient tensor in turbulent flows}},
  author={Wallace, J. M. and Vukoslav{\v{c}}evi{\'c}, P. V.},
  journal={Annu. Rev. Fluid Mech.},
  volume={42},
  pages={157--181},
  year={2010},
  publisher={Annual Reviews}
}

@article{meneveau2011,
  title={{Lagrangian dynamics and models of the velocity gradient tensor in turbulent flows}},
  author={Meneveau, C.},
  journal={Annu. Rev. Fluid Mech.},
  volume={43},
  pages={219--245},
  year={2011},
  publisher={Annual Reviews}
}

@article{vukoslav2009,
 author={Vukoslavcevic, V. and Beratlis, N. and Balaras, E. and Wallace, J. M. and Sun, O.},
 title={{On the spatial resolution of velocity and velocity gradient-based turbulence statistics measured with multi-sensor hot-wire probes}},
 journal={Exp. Fluids},
 pages={109},
 year={2009}
}

@article{das2002,
  title={The surprise element: jumps in interest rates},
  author={Das, S. R.},
  journal={J. Econometrics},
  volume={106},
  pages={27--65},
  year={2002},
  publisher={Elsevier}
}

@article{giraudo1997,
  title={{Jump-diffusion processes as models for neuronal activity}},
  author={Giraudo, M. T. and Sacerdote, L.},
  journal={Biosystems},
  volume={40},
  pages={75--82},
  year={1997},
  publisher={Elsevier}
}

@incollection{sacerdote2013,
  title={Stochastic integrate and fire models: a review on mathematical methods and their applications},
  author={Sacerdote, L. and Giraudo, M. T.},
  booktitle={Stoc. Biomath. Models},
  pages={99--148},
  year={2013},
  publisher={Springer}
}
% is this abbreviation correct?

@article{patel2008,
  title={{Stochastic resonance in continuous and spiking neuron models with Levy noise}},
  author={Patel, A. and Kosko, B.},
  journal={IEEE T. Neural Networks},
  volume={19},
  pages={1993--2008},
  year={2008},
  publisher={IEEE}
}

% Finances, First Jump Model
@article{cox1976,
  title={{The valuation of options for alternative stochastic processes}},
  author={Cox, J. C. and Ross, S. A.},
  journal={J. Financ. Econ.},
  volume={3},
  pages={145--166},
  year={1976},
  publisher={Elsevier}
}

% Finances, First Jump-Diffusion Model
@article{merton1976,
  title={{Option pricing when underlying stock returns are discontinuous}},
  author={Merton, R. C.},
  journal={J. Financ. Econ.},
  volume={3},
  pages={125--144},
  year={1976},
  publisher={Elsevier}
}

% Finances, Jump-Diffusion
@article{ball1993,
  title={{A jump diffusion model for the European Monetary System}},
  author={Ball, C. A. and Roma, A.},
  journal={J. Int. Money Financ.},
  volume={12},
  pages={475--492},
  year={1993},
  publisher={Elsevier}
}

@article{duffie2000,
  title={{Transform analysis and asset pricing for affine jump-diffusions}},
  author={Duffie, D. and Pan, J. and Singleton, K.},
  journal={Econometrica},
  volume={68},
  pages={1343--1376},
  year={2000},
  publisher={Wiley Online Library}
}

% Physics, Jump-Diffusion
@article{chudley1961,
  title={{Neutron scattering from a liquid on a jump diffusion model}},
  author={Chudley, C. T. and Elliott, R. J.},
  journal={P. Phys. Soc.},
  volume={77},
  pages={353},
  year={1961},
  publisher={IOP Publishing}
}

@article{funke1993,
  title={Jump relaxation in solid electrolytes},
  author={Funke, K.},
  journal={Prog. Solid State Ch.},
  volume={22},
  pages={111--195},
  year={1993},
  publisher={Elsevier}
}

@article{ellis1993,
  title={{Observation of jump diffusion of isolated sodium atoms on a Cu (001) surface by Helium atom scattering}},
  author={Ellis, J. and Toennies, J. P.},
  journal={Phys. Rev. Lett.},
  volume={70},
  pages={2118},
  year={1993},
  publisher={APS}
}

@article{montalenti1999,
  title={{Jumps and concerted moves in Cu, Ag, and Au (110) adatom self-diffusion}},
  author={Montalenti, F. and Ferrando, R.},
  journal={Phys. Rev. B},
  volume={59},
  pages={5881},
  year={1999},
  publisher={APS}
}

% Biomedicine, Jump-diffusion
@article{grenander1994,
  title={{Representations of knowledge in complex systems}},
  author={Grenander, U. and Miller, M. I.},
  journal={J. Roy. Stat. Soc. B Met.},
  volume={56},
  pages={549--581},
  year={1994},
  publisher={Wiley Online Library}
}

% Image recognition, jump-diffusion

@article{srivastava2002,
  title={{Jump--diffusion Markov processes on orthogonal groups for object pose estimation}},
  author={Srivastava, A. and Grenander, U. and Jensen, G. R. and Miller, M. I.},
  journal={J. Stat. Plan. Infer.},
  volume={103},
  pages={15--37},
  year={2002},
  publisher={Elsevier}
}

%%%%% Measure of Lagrangian Intermittency Parameter

@article{huang2014,
  title={{La\-gran\-gian cas\-ca\-de in three-dimensional ho\-mo\-ge\-neous and isotropic turbulence}},
  author={Huang, Y. and Schmitt, F. G.},
  journal={J. Fluid Mech.},
  volume={741},
  year={2014},
  publisher={Cambridge University Press}
}

%%%%% First Generation Cascade Models

@article{novikov1964,
  title={{The intermittency of turbulence and the spectrum of energy dissipation fluctuations}},
  author={Novikov, E. A. and Stewart, R. W.},
  journal={Izv. Geophys. Ser},
  volume={3},
  pages={408--413},
  year={1964}
}

@article{frisch1978,
  title={{A simple dynamical model of intermittent fully developed turbulence}},
  author={Frisch, U. and Sulem, P.-L. and Nelkin, M.},
  journal={J. Fluid Mech.},
  volume={87},
  pages={719--736},
  year={1978},
  publisher={Cambridge University Press}
}

@article{schertzer1984,
  title={{On the dimension of atmospheric motions}},
  author={Schertzer, D. and Lovejoy, S.},
  journal={Turbulence and Chaotic phenomena in Fluids},
  pages={505--512},
  year={1984},
  publisher={North-Holland}
}

@article{benzi1984,
  title={{On the multifractal nature of fully developed turbulence and chaotic systems}},
  author={Benzi, R. and Paladin, G. and Parisi, G. and Vulpiani, A.},
  journal={J. Phys. A},
  volume={17},
  pages={3521},
  year={1984},
  publisher={IOP Publishing}
}

@article{vainshtein1994,
  title={{Scaling exponents for turbulence and other random processes and their relationships with multifractal structure}},
  author={Vainshtein, S. I. and Sreenivasan, K. R. and Pierrehumbert, R. T. and Kashyap, V. and Juneja, A.},
  journal={Phys. Rev. E},
  volume={50},
  pages={1823},
  year={1994},
  publisher={APS}
}

@article{muzy2002,
  title={{Multifractal stationary random measures and multifractal random walks with log infinitely divisible scaling laws}},
  author={Muzy, J.-F. and Bacry, E.},
  journal={Phys. Rev. E},
  volume={66},
  pages={056121},
  year={2002},
  publisher={APS}
}

@article{muzy1994,
  title={{The multifractal formalism revisited with wavelets}},
  author={Muzy, J.-F. and Bacry, E. and Arneodo, A.},
  journal={Int. J. Bifurcat. Chaos},
  volume={4},
  pages={245--302},
  year={1994},
  publisher={World Scientific}
}

@article{ashurst1987,
  title={{Alignment of vorticity and scalar gradient with strain rate in simulated Navier--Stokes turbulence}},
  author={Ashurst, W. T. and Kerstein, A. R. and Kerr, R. M. and Gibson, C. H.},
  journal={Phys. Fluids},
  volume={30},
  pages={2343--2353},
  year={1987},
  publisher={AIP}
}

@article{kailasnath1992,
  title={{Probability density of velocity increments in turbulent flows}},
  author={Kailasnath, P. and Sreenivasan, K. R. and Stolovitzky, G.},
  journal={Phys. Rev. Lett.},
  volume={68},
  pages={2766},
  year={1992},
  publisher={APS}
}


@article{schumacher2014,
  title={{Small-scale universality in fluid turbulence}},
  author={Schumacher, J. and Scheel, J. D. and Krasnov, D. and Donzis, D. A. and Yakhot, V. and Sreenivasan, K. R.},
  journal={P. Natl. Acad. Sci. USA},
  volume={111},
  pages={10961--10965},
  year={2014},
  publisher={National Acad Sciences}
}

@article{benzi1991,
  title={{Multifractality in the statistics of the velocity gradients in turbulence}},
  author={Benzi, R. and Biferale, L. and Paladin, G. and Vulpiani, A. and Vergassola, M.},
  journal={Phys. Rev. Lett.},
  volume={67},
  pages={2299},
  year={1991},
  publisher={APS}
}

@article{biferale1993,
  title={{Probability distribution functions in turbulent flows and shell models}},
  author={Biferale, L.},
  journal={Phys. Fluids A},
  volume={5},
  pages={428--435},
  year={1993},
  publisher={AIP}
}

@article{castaing1990,
  title={{Velocity probability density functions of high Reynolds number turbulence}},
  author={Castaing, B. and Gagne, Y. and Hopfinger, E. J.},
  journal={Physica D},
  volume={46},
  pages={177--200},
  year={1990},
  publisher={Elsevier}
}

@article{gurvitch1963,
  title={On the experimental evaluation of the fluctuations of dissipation of turbulent energy},
  author={Gurvitch, A. S. and Zubkovski, S. L.},
  year={1963},
  journal={Izv. An. SSSR Geol.+},
  volume={12},
  pages={1856-1858}
  }
% Izv. Akad. Nauk. SSSR Ser. Geofiz.
% Izvestia, Geophysics Series (following the reference in Some Physical and Statistical Aspects of Clear Air Turbulence, Peter F. Lester)

@article{pond1965,
  title={Measurements of the statistical characteristics of small-scale turbulent motions},
  author={Pond, S. and Stewart, R. W.},
  year={1965},
  journal={Izv. An. SSSR Fiz. Atm.+},
  volume={1},
  page={914}
  }
% Styuart, he is Russian
% https://books.google.com.br/books?id=3U8qAAAAMAAJ&lpg=RA3-PA134&ots=r0g6BcZ-CV&dq=pond%20stewart%20izvestiya&pg=RA3-PA134#v=onepage&q=pond%20stewart%20izvestiya&f=false

@article{mandelbrot1974,
  title={Intermittent turbulence in self-similar cascades: divergence of high moments and dimension of the carrier},
  author={Mandelbrot, B. B.},
  journal={J. Fluid Mech.},
  volume={62},
  pages={331--358},
  year={1974},
  publisher={Cambridge University Press}
}

@article{schmitt2001,
  title={Stochastic equations generating continuous multiplicative cascades},
  author={Schmitt, F. G. and Marsan, D.},
  journal={Eur. Phys. J. B},
  volume={20},
  pages={3--6},
  year={2001},
  publisher={Springer}
}

@inproceedings{yaglom1966,
  title={The influence of fluctuations in energy dissipation on the shape of turbulence characteristics in the inertial interval},
  author={Yaglom, A. M.},
  booktitle={Sov. Phys. Dokl.},
  volume={11},
  pages={26},
  year={1966}
}

@article{yeungpope1989,
  title={Lagrangian statistics from direct numerical simulations of isotropic turbulence},
  author={Yeung, P. K. and Pope, S. B.},
  journal={J. Fluid Mech.},
  volume={207},
  pages={531--586},
  year={1989},
  publisher={Cambridge University Press}
}

@article{barralmandelbrot2002,
  title={Multifractal products of cylindrical pulses},
  author={Barral, J. and Mandelbrot, B. B.},
  journal={Probab. Theory Rel.},
  volume={124},
  number={3},
  pages={409--430},
  year={2002},
  publisher={Springer}
}

@article{schmittmarsan2001,
  title={Stochastic equations generating continuous multiplicative cascades},
  author={Schmitt, F. G. and Marsan, D.},
  journal={Eur. Phys. J. B},
  volume={20},
  pages={3--6},
  year={2001},
  publisher={Springer}
}

@article{arneodo1998prl,
  title={Analysis of random cascades using space-scale correlation functions},
  author={Arneodo, A. and Bacry, E. and Manneville, S. and Muzy, J.-F.},
  journal={Phys. Rev. Lett.},
  volume={80},
  pages={708},
  year={1998},
  publisher={APS}
}

@article{arneodo1998jmathphys,
  title={Random cascades on wavelet dyadic trees},
  author={Arneodo, A. and Bacry, E. and Muzy, J.-F.},
  journal={J. Math. Phys},
  volume={39},
  pages={4142--4164},
  year={1998},
  publisher={AIP}
}

@article{schertzer1987,
  title={Physical modeling and analysis of rain and clouds by anisotropic scaling multiplicative processes},
  author={Schertzer, D. and Lovejoy, S.},
  journal={J. Geophys. Res.-Atmos.},
  volume={92},
  pages={9693--9714},
  year={1987},
  publisher={Wiley Online Library}
}

@incollection{schertzer1991,
  author={Schertzer, D. and Lovejoy, S.},
  booktitle={Scaling, fractals and non-linear variability in geophysics},
  pages={41},
  year={1991},
  publisher={Kluwer, Berlin}
}

@article{bacry2001,
  title={Multifractal random walk},
  author={Bacry, E. and Delour, J. and Muzy, J.-F.},
  journal={Phys. Rev. E},
  volume={64},
  pages={026103},
  year={2001},
  publisher={APS}
}

@article{duplantier2014,
  title={Liouville quantum gravity as a mating of trees},
  author={Duplantier, B. and Miller, J. and Sheffield, S.},
  journal={arXiv preprint arXiv:1409.7055},
  year={2014}
}

@article{fyodorov2014,
  title={Freezing transitions and extreme values: random matrix theory, and disordered landscapes},
  author={Fyodorov, Y. V. and Keating, J. P.},
  journal={Philos. T. R. Soc. A},
  volume={372},
  pages={20120503},
  year={2014},
  publisher={The Royal Society Publishing.}
}

@article{duchon2012,
  title={Forecasting volatility with the multifractal random walk model},
  author={Duchon, J. and Robert, R. and Vargas, V.},
  journal={Math. Financ.},
  volume={22},
  pages={83--108},
  year={2012},
  publisher={Wiley Online Library}
}

@article{ripley1990,
  title={Finding spiral structures in images of galaxies},
  author={Ripley, B. D. and Sutherland, A. L.},
  journal={Philos. T. Roy. Soc. A},
  volume={332},
  pages={477--485},
  year={1990},
  publisher={The Royal Society London}
}

% particles / spheroids in turbulence
@article{zhao2015,
  title={Rotation of nonspherical particles in turbulent channel flow},
  author={Zhao, L. and Challabotla, N. R. and Andersson, H. I. and Variano, E.},
  journal={Phys. Rev. Lett.},
  volume={115},
  number={24},
  pages={244501},
  year={2015},
  publisher={APS}
}

@article{challabotla2015,
  title={Orientation and rotation of inertial disk particles in wall turbulence},
  author={Challabotla, N. R. and Zhao, L. and Andersson, H. I.},
  journal={J. Fluid Mech.},
  volume={766},
  year={2015},
  publisher={Cambridge University Press}
}

@article{byron2015,
  title={Shape-dependence of particle rotation in isotropic turbulence},
  author={Byron, M. and Einarsson, J. and Gustavsson, K. and Voth, G. and Mehlig, B. and Variano, E.},
  journal={Phys. Fluids},
  volume={27},
  pages={035101},
  year={2015},
  publisher={AIP Publishing LLC}
}

@article{gustavsson2014,
  title={Tumbling of small axisymmetric particles in random and turbulent flows},
  author={Gustavsson, K. and Einarsson, J. and Mehlig, B.},
  journal={Phys. Rev. Lett.},
  volume={112},
  pages={014501},
  year={2014},
  publisher={APS}
}

@article{parsa2012,
  title={Rotation rate of rods in turbulent fluid flow},
  author={Parsa, S. and Calzavarini, E. and Toschi, F. and Voth, G.},
  journal={Phys. Rev. Lett.},
  volume={109},
  number={13},
  pages={134501},
  year={2012},
  publisher={APS}
}

% experiments, structures and intermittency
@article{debue2018prf,
  title={{Experimental test of the crossover between the inertial and the dissipative range in a turbulent swirling flow}},
  author={Debue, P. and Kuzzay, D. and Saw, E.-W. and Daviaud, F. and Dubrulle, B. and Canet, L. and Rossetto, V. and Wschebor, N.},
  journal={Phys. Rev. Fluids},
  volume={3},
  pages={024602},
  year={2018},
  publisher={APS}
}

@article{debue2018pre,
  title={Dissipation, intermittency, and singularities in incompressible turbulent flows},
  author={Debue, P. and Shukla, V. and Kuzzay, D. and Faranda, D. and Saw, E.-W. and Daviaud, F. and Dubrulle, B.},
  journal={Phys. Rev. E},
  volume={97},
  pages={053101},
  year={2018},
  publisher={APS}
}

@article{barjona2017,
  title={{Kolmogorov's Lagrangian similarity law revisited}},
  author={Barjona, M. and da Silva, C. B.},
  journal={Phys. Fluids},
  volume={29},
  pages={105106},
  year={2017},
  publisher={AIP Publishing LLC}
}

@article{bacry2008,
  title={{Log-Normal continuous cascades: aggregation properties and estimation. Application to financial time-series}},
  author={Bacry, E. and Kozhemyak, A. and Muzy, J.-F.},
  journal={arXiv preprint arXiv:0804.0185},
  year={2008}
}

@article{muzy2000,
  title={Modelling fluctuations of financial time series: from cascade process to stochastic volatility model},
  author={Muzy, J.-F. and Delour, J. and Bacry, E.},
  journal={Eur. Phys. J. B},
  volume={17},
  number={3},
  pages={537--548},
  year={2000},
  publisher={Springer}
}

@book{bouchaud2003,
  title={Theory of financial risk and derivative pricing: from statistical physics to risk management},
  author={Bouchaud, J.-P. and Potters, M.},
  year={2003},
  publisher={Cambridge university press}
}

@article{mandelbrot1997,
  title={A multifractal model of asset returns},
  author={Mandelbrot, B. B. and Fisher, A. J. and Calvet, L. E.},
  year={1997},
  publisher={Cowles Foundation}
}

@article{ghashghaie1996,
  title={Turbulent cascades in foreign exchange markets},
  author={Ghashghaie, S. and Breymann, W. and Peinke, J. and Talkner, P. and Dodge, Y.},
  journal={Nature},
  volume={381},
  pages={767--770},
  year={1996},
  publisher={Nature Publishing Group}
}

@article{coles1991,
  title={A lognormal model for the cosmological mass distribution},
  author={Coles, P. and Jones, B.},
  journal={Mon. Not. R. Astron. Soc.},
  volume={248},
  pages={1--13},
  year={1991},
  publisher={The Royal Astronomical Society}
}

@article{frankot1987, 
  title={Lognormal random-field models and their applications to radar image synthesis},
  author={Frankot, R. T. and Chellappa, R.},
  journal={IEEE T. Geosci. Remote},
  pages={195--207},
  year={1987},
  publisher={IEEE}
}

@article{andersen2007,
  title={{Roughing it up: Including jump components in the measurement, modeling, and forecasting of return volatility}},
  author={Andersen, T. G. and Bollerslev, T. and Diebold, F. X.},
  journal={Rev. Econ. Statistics},
  volume={89},
  pages={701--720},
  year={2007},
  publisher={MIT Press}
}

@article{benzi2009,
  title={{Velocity-gradient statistics along particle trajectories in turbulent flows: The refined similarity hypothesis in the Lagrangian frame}},
  author={Benzi, R. and Biferale, L. and Calzavarini, E. and Lohse, D. and Toschi, F.},
  journal={Phys. Rev. E},
  volume={80},
  pages={066318},
  year={2009},
  publisher={APS}
}

@article{yeung2002,
  title={Lagrangian investigations of turbulence},
  author={Yeung, P. K.},
  journal={Annu. Rev. Fluid Mech.},
  volume={34},
  pages={115--142},
  year={2002},
  publisher={Annual Reviews}
}

@article{sawfordyeung2011,
  title={{Kolmogorov similarity scaling for one-particle Lagrangian statistics}},
  author={Sawford, B. L. and Yeung, P. K.},
  journal={Phys. Fluids},
  volume={23},
  pages={091704},
  year={2011},
  publisher={American Institute of Physics}
}

% small scale turbulence, long range correlations
@article{sreenivasanantonia1997,
  title={The phenomenology of small-scale turbulence},
  author={Sreenivasan, K. R. and Antonia, R. A.},
  journal={Annu. Rev. Fluid Mech.},
  volume={29},
  pages={435--472},
  year={1997},
  publisher={Annual Reviews}
}

@article{meneveausreenivasan1991,
  title={The multifractal nature of turbulent energy dissipation},
  author={Meneveau, C. and Sreenivasan, K. R.},
  journal={J. Fluid Mech.},
  volume={224},
  pages={429--484},
  year={1991},
  publisher={Cambridge University Press}
}

@article{gurvichyaglom1967,
  title={Breakdown of eddies and probability distributions for small-scale turbulence},
  author={Gurvich, A. S. and Yaglom, A. M.},
  journal={Phys. Fluids},
  volume={10},
  pages={S59--S65},
  year={1967},
  publisher={American Institute of Physics}
}

@article{motoori2019,
  title={Generation mechanism of a hierarchy of vortices in a turbulent boundary layer},
  author={Motoori, Y. and Goto, S.},
  journal={J. Fluid Mech.},
  volume={865},
  pages={1085--1109},
  year={2019},
  publisher={Cambridge University Press}
}

@article{doan2018,
  title={Scale locality of the energy cascade using real space quantities},
  author={Doan, N. A. K. and Swaminathan, N. and Davidson, P. A. and Tanahashi, M.},
  journal={Phys. Rev. Fluids},
  volume={3},
  pages={084601},
  year={2018},
  publisher={APS}
}

@article{lejan1997,
  title={Stochastic cascades and 3-dimensional Navier--Stokes equations},
  author={Le Jan, Y. and Sznitman, A. S.},
  journal={Probab. Theory Rel.},
  volume={109},
  pages={343--366},
  year={1997},
  publisher={Springer}
}

% volatility is lognormal and long range correlated
@article{liu1999,
  title={Statistical properties of the volatility of price fluctuations},
  author={Liu, Y. and Gopikrishnan, P. and Stanley, H. E.},
  journal={Phys. Rev. E},
  volume={60},
  pages={1390},
  year={1999},
  publisher={APS}
}

% cond mat multifractal
@article{kravtsov1997,
  title={New class of random matrix ensembles with multifractal eigenvectors},
  author={Kravtsov, V. E. and Muttalib, K. A.},
  journal={Phys. Rev. Lett.},
  volume={79},
  pages={1913},
  year={1997},
  publisher={APS}
}

@article{serbyn2017,
  title={Thouless energy and multifractality across the many-body localization transition},
  author={Serbyn, M. and Papi{\'c}, Z. and Abanin, D. A.},
  journal={Phys. Rev. B},
  volume={96},
  pages={104201},
  year={2017},
  publisher={APS}
}

@article{schmitt1994,
  author = {Schmitt, F. G. and Schertzer, D. and Lovejoy, S. and Brunet, Y.},
  title = {Empirical study of multifractal phase transitions in atmospheric turbulence},
  journal = {Nonlinear Proc. Geoph.},
  volume = {1},
  year = {1994},
  pages = {95--104},
}

@article{lashermes2004,
  title={New insights into the estimation of scaling exponents},
  author={Lashermes, B. and Abry, P. and Chainais, P.},
  journal={Int. J. Wavelets Multi.},
  volume={2},
  pages={497--523},
  year={2004},
  publisher={World Scientific}
}

% Euler intermittency parameter measures
@article{stolovitzky1992,
  title={Kolmogorov's refined similarity hypotheses},
  author={Stolovitzky, G. and Kailasnath, P. and Sreenivasan, K. R.},
  journal={Phys. Rev. Lett.},
  volume={69},
  pages={1178},
  year={1992},
  publisher={APS}
}


@article{stolovitzky1994,
  title={Kolmogorov's refined similarity hypotheses for turbulence and general stochastic processes},
  author={Stolovitzky, G. and Sreenivasan, K. R.},
  journal={Rev. Mod. Phys.},
  volume={66},
  pages={229},
  year={1994},
  publisher={APS}
}

@article{praskovsky1997,
  title={Further experimental support for the Kolmogorov refined similarity hypothesis},
  author={Praskovsky, A. and Praskovskaya, E. and Horst, T.},
  journal={Phys. Fluids},
  volume={9},
  pages={2465--2467},
  year={1997},
  publisher={American Institute of Physics}
}

@article{chen1997,
  title={Refined similarity hypothesis for transverse structure functions in fluid turbulence},
  author={Chen, S. and Sreenivasan, K. R. and Nelkin, M. and Cao, N.},
  journal={Phys. Rev. Lett.},
  volume={79},
  number={12},
  pages={2253},
  year={1997},
  publisher={APS}
}

@article{borgas1993,
  title={{The multifractal Lagrangian nature of turbulence}},
  author={Borgas, M. S.},
  journal={Philos. T. Roy. Soc. A},
  volume={342},
  pages={379--411},
  year={1993},
  publisher={The Royal Society London}
}

@article{pereira2016,
  title={A dissipative random velocity field for fully developed fluid turbulence},
  author={Pereira, R. M. and Garban, C. and Chevillard, L.},
  journal={J. Fluid Mech.},
  volume={794},
  pages={369--408},
  year={2016},
  publisher={Cambridge University Press}
}

@article{morgado2016,
  title={{Thermostatistics of small nonlinear systems: Poissonian athermal bath}},
  author={Morgado, W. A. M. and Queir{\'o}s, S. M. D.},
  journal={Phys. Rev. E},
  volume={93},
  pages={012121},
  year={2016},
  publisher={APS}
}

@article{mandelbrot1974paris,
  title={Multiplications al{\'e}atoires it{\'e}r{\'e}es et distributions invariantes par moyenne pond{\'e}r{\'e}e al{\'e}atoire},
  author={Mandelbrot, B. B.},
  journal={C. R. Acad. Sci. Paris},
  volume={278},
  pages={355--358},
  year={1974}
}

@article{wiener1938,
  title={The homogeneous chaos},
  author={Wiener, N.},
  journal={Am. J. Math.},
  volume={60},
  pages={897--936},
  year={1938},
  publisher={JSTOR}
}

@article{blatman2011,
  title={Adaptive sparse polynomial chaos expansion based on least angle regression},
  author={Blatman, G. and Sudret, B.},
  journal={J. Comp. Phys.},
  volume={230},
  pages={2345--2367},
  year={2011},
  publisher={Elsevier}
}

@book{temam2001,
  title={Navier-Stokes equations: theory and numerical analysis},
  author={Temam, R.},
  volume={343},
  year={2001},
  publisher={American Mathematical Soc.}
}

@article{shen2007,
  title={A kinetic-theory based first order slip boundary condition for gas flow},
  author={Shen, S. and Chen, G. and Crone, R. M. and Anaya-Dufresne, M.},
  journal={Phys. Fluids},
  volume={19},
  pages={086101},
  year={2007},
  publisher={American Institute of Physics}
}

@article{denniston2006,
  title={General continuum boundary conditions for miscible binary fluids from molecular dynamics simulations},
  author={Denniston, C. and Robbins, M. O.},
  journal={J. Chem. Phys.},
  volume={125},
  pages={214102},
  year={2006},
  publisher={American Institute of Physics}
}

@article{arenas2010,
  title={Functional integral approach for multiplicative stochastic processes},
  author={Arenas, Z. G. and Barci, D. G.},
  journal={Phys. Rev. E},
  volume={81},
  pages={051113},
  year={2010},
  publisher={APS}
}

@article{janssen1992,
  title={From Phase Transitions to Chaos},
  author={Janssen, H. K.},
  journal={Topics in Modern Statistical Physics},
  year={1992},
  publisher={World Scientific Singapore}
}

